What Makes a Level Hard in Super Mario Maker 2?

Games like Super Mario Maker 2 (SMM2) lower the barrier for casual users to become level designers. In this paper, we set out to analyze a vast amount of data about SMM2 user-written levels, in order to understand what factors affect a level's difficulty as experienced by other users. To this end, we perform two kinds of analyses: one based on regression models and one using natural language processing techniques. The main results shed light on which level characteristics (e.g., its style, popularity, timing) and which topics and sentiments have a consistent association with easier or harder levels. While none of our findings are startling, they help distill some key differences between easy and hard SMM2 levels, which, in turn, can pave the way for a better understanding of end-user level design.

==> floats/stats.tex <==
\pgfkeyssetvalue{/sea/N.raw.vars}{36}
\pgfkeyssetvalue{/sea/N.all.variables}{22}
\pgfkeyssetvalue{/sea/N.levels}{26609725}
\pgfkeyssetvalue{/sea/N.fml.all.variables}{13}
\pgfkeyssetvalue{/sea/N.fml.all.clears.variables}{14}
\pgfkeyssetvalue{/sea/N.fml.all.attempts.variables}{14}
\pgfkeyssetvalue{/sea/N.fml.all.both.variables}{15}
\pgfkeyssetvalue{/sea/N.all.user.vars}{19}
\pgfkeyssetvalue{/sea/N.users}{5935222}
\pgfkeyssetvalue{/sea/N.all.makers}{2635933}
\pgfkeyssetvalue{/sea/N.fml.user.all.variables}{28}
\pgfkeyssetvalue{/sea/N.user.vars}{28}
\pgfkeyssetvalue{/sea/aic:user/fml.all.both}{-31284103.9032247}
\pgfkeyssetvalue{/sea/aic:user/fml.user.all}{-31664107.3053527}
\pgfkeyssetvalue{/sea/resdev:user/fml.all.both}{480817.654006252}
\pgfkeyssetvalue{/sea/resdev:user/fml.user.all}{473999.540342909}
\pgfkeyssetvalue{/sea/numeric/min:world_record}{-0.001}
\pgfkeyssetvalue{/sea/numeric/min:upload_time}{0.015}
\pgfkeyssetvalue{/sea/numeric/min:upload_attempts}{1}
\pgfkeyssetvalue{/sea/numeric/min:num_comments}{0}
\pgfkeyssetvalue{/sea/numeric/min:timer}{10}
\pgfkeyssetvalue{/sea/numeric/min:autoscroll_speed}{0}
\pgfkeyssetvalue{/sea/numeric/min:clears}{0}
\pgfkeyssetvalue{/sea/numeric/min:attempts}{0}
\pgfkeyssetvalue{/sea/numeric/min:clear_rate_p}{0}
\pgfkeyssetvalue{/sea/numeric/min:likes}{0}
\pgfkeyssetvalue{/sea/numeric/min:boos}{0}
\pgfkeyssetvalue{/sea/numeric/min:unique_players_and_versus}{0}
\pgfkeyssetvalue{/sea/numeric/min:courses_played}{0}
\pgfkeyssetvalue{/sea/numeric/min:courses_cleared}{0}
\pgfkeyssetvalue{/sea/numeric/min:courses_attempted}{0}
\pgfkeyssetvalue{/sea/numeric/min:courses_deaths}{0}
\pgfkeyssetvalue{/sea/numeric/min:likes_maker}{0}
\pgfkeyssetvalue{/sea/numeric/min:maker_points}{0}
\pgfkeyssetvalue{/sea/numeric/min:easy_highscore}{0}
\pgfkeyssetvalue{/sea/numeric/min:normal_highscore}{0}
\pgfkeyssetvalue{/sea/numeric/min:expert_highscore}{0}
\pgfkeyssetvalue{/sea/numeric/min:super_expert_highscore}{0}
\pgfkeyssetvalue{/sea/numeric/min:versus_rating}{0}
\pgfkeyssetvalue{/sea/numeric/min:first_clears}{0}
\pgfkeyssetvalue{/sea/numeric/min:world_records}{0}
\pgfkeyssetvalue{/sea/numeric/min:uploaded_levels}{0}
\pgfkeyssetvalue{/sea/numeric/25p:world_record}{9.836}
\pgfkeyssetvalue{/sea/numeric/25p:upload_time}{21.899}
\pgfkeyssetvalue{/sea/numeric/25p:upload_attempts}{1}
\pgfkeyssetvalue{/sea/numeric/25p:num_comments}{0}
\pgfkeyssetvalue{/sea/numeric/25p:timer}{300}
\pgfkeyssetvalue{/sea/numeric/25p:autoscroll_speed}{0}
\pgfkeyssetvalue{/sea/numeric/25p:clears}{4}
\pgfkeyssetvalue{/sea/numeric/25p:attempts}{22}
\pgfkeyssetvalue{/sea/numeric/25p:clear_rate_p}{0.0958466453674121}
\pgfkeyssetvalue{/sea/numeric/25p:likes}{0}
\pgfkeyssetvalue{/sea/numeric/25p:boos}{0}
\pgfkeyssetvalue{/sea/numeric/25p:unique_players_and_versus}{10}
\pgfkeyssetvalue{/sea/numeric/25p:courses_played}{127}
\pgfkeyssetvalue{/sea/numeric/25p:courses_cleared}{80}
\pgfkeyssetvalue{/sea/numeric/25p:courses_attempted}{508}
\pgfkeyssetvalue{/sea/numeric/25p:courses_deaths}{376}
\pgfkeyssetvalue{/sea/numeric/25p:likes_maker}{23}
\pgfkeyssetvalue{/sea/numeric/25p:maker_points}{780}
\pgfkeyssetvalue{/sea/numeric/25p:easy_highscore}{6}
\pgfkeyssetvalue{/sea/numeric/25p:normal_highscore}{0}
\pgfkeyssetvalue{/sea/numeric/25p:expert_highscore}{0}
\pgfkeyssetvalue{/sea/numeric/25p:super_expert_highscore}{0}
\pgfkeyssetvalue{/sea/numeric/25p:versus_rating}{0}
\pgfkeyssetvalue{/sea/numeric/25p:first_clears}{1}
\pgfkeyssetvalue{/sea/numeric/25p:world_records}{0}
\pgfkeyssetvalue{/sea/numeric/25p:uploaded_levels}{10}
\pgfkeyssetvalue{/sea/numeric/50p:world_record}{21.032}
\pgfkeyssetvalue{/sea/numeric/50p:upload_time}{42.361}
\pgfkeyssetvalue{/sea/numeric/50p:upload_attempts}{1}
\pgfkeyssetvalue{/sea/numeric/50p:num_comments}{0}
\pgfkeyssetvalue{/sea/numeric/50p:timer}{300}
\pgfkeyssetvalue{/sea/numeric/50p:autoscroll_speed}{0}
\pgfkeyssetvalue{/sea/numeric/50p:clears}{10}
\pgfkeyssetvalue{/sea/numeric/50p:attempts}{54}
\pgfkeyssetvalue{/sea/numeric/50p:clear_rate_p}{0.25}
\pgfkeyssetvalue{/sea/numeric/50p:likes}{1}
\pgfkeyssetvalue{/sea/numeric/50p:boos}{1}
\pgfkeyssetvalue{/sea/numeric/50p:unique_players_and_versus}{21}
\pgfkeyssetvalue{/sea/numeric/50p:courses_played}{342}
\pgfkeyssetvalue{/sea/numeric/50p:courses_cleared}{219}
\pgfkeyssetvalue{/sea/numeric/50p:courses_attempted}{1397}
\pgfkeyssetvalue{/sea/numeric/50p:courses_deaths}{1064}
\pgfkeyssetvalue{/sea/numeric/50p:likes_maker}{71}
\pgfkeyssetvalue{/sea/numeric/50p:maker_points}{1599}
\pgfkeyssetvalue{/sea/numeric/50p:easy_highscore}{29}
\pgfkeyssetvalue{/sea/numeric/50p:normal_highscore}{0}
\pgfkeyssetvalue{/sea/numeric/50p:expert_highscore}{0}
\pgfkeyssetvalue{/sea/numeric/50p:super_expert_highscore}{0}
\pgfkeyssetvalue{/sea/numeric/50p:versus_rating}{308}
\pgfkeyssetvalue{/sea/numeric/50p:first_clears}{4}
\pgfkeyssetvalue{/sea/numeric/50p:world_records}{2}
\pgfkeyssetvalue{/sea/numeric/50p:uploaded_levels}{25}
\pgfkeyssetvalue{/sea/numeric/75p:world_record}{43.85}
\pgfkeyssetvalue{/sea/numeric/75p:upload_time}{77.423}
\pgfkeyssetvalue{/sea/numeric/75p:upload_attempts}{4}
\pgfkeyssetvalue{/sea/numeric/75p:num_comments}{1}
\pgfkeyssetvalue{/sea/numeric/75p:timer}{300}
\pgfkeyssetvalue{/sea/numeric/75p:autoscroll_speed}{0}
\pgfkeyssetvalue{/sea/numeric/75p:clears}{28}
\pgfkeyssetvalue{/sea/numeric/75p:attempts}{127}
\pgfkeyssetvalue{/sea/numeric/75p:clear_rate_p}{0.5}
\pgfkeyssetvalue{/sea/numeric/75p:likes}{4}
\pgfkeyssetvalue{/sea/numeric/75p:boos}{2}
\pgfkeyssetvalue{/sea/numeric/75p:unique_players_and_versus}{48}
\pgfkeyssetvalue{/sea/numeric/75p:courses_played}{840}
\pgfkeyssetvalue{/sea/numeric/75p:courses_cleared}{534}
\pgfkeyssetvalue{/sea/numeric/75p:courses_attempted}{3391}
\pgfkeyssetvalue{/sea/numeric/75p:courses_deaths}{2654}
\pgfkeyssetvalue{/sea/numeric/75p:likes_maker}{174}
\pgfkeyssetvalue{/sea/numeric/75p:maker_points}{2441}
\pgfkeyssetvalue{/sea/numeric/75p:easy_highscore}{100}
\pgfkeyssetvalue{/sea/numeric/75p:normal_highscore}{4}
\pgfkeyssetvalue{/sea/numeric/75p:expert_highscore}{1}
\pgfkeyssetvalue{/sea/numeric/75p:super_expert_highscore}{0}
\pgfkeyssetvalue{/sea/numeric/75p:versus_rating}{1865}
\pgfkeyssetvalue{/sea/numeric/75p:first_clears}{11}
\pgfkeyssetvalue{/sea/numeric/75p:world_records}{7}
\pgfkeyssetvalue{/sea/numeric/75p:uploaded_levels}{52}
\pgfkeyssetvalue{/sea/numeric/99p:world_record}{258.211759999998}
\pgfkeyssetvalue{/sea/numeric/99p:upload_time}{261.384}
\pgfkeyssetvalue{/sea/numeric/99p:upload_attempts}{45}
\pgfkeyssetvalue{/sea/numeric/99p:num_comments}{13}
\pgfkeyssetvalue{/sea/numeric/99p:timer}{500}
\pgfkeyssetvalue{/sea/numeric/99p:autoscroll_speed}{0}
\pgfkeyssetvalue{/sea/numeric/99p:clears}{247}
\pgfkeyssetvalue{/sea/numeric/99p:attempts}{1431}
\pgfkeyssetvalue{/sea/numeric/99p:clear_rate_p}{1}
\pgfkeyssetvalue{/sea/numeric/99p:likes}{49}
\pgfkeyssetvalue{/sea/numeric/99p:boos}{15}
\pgfkeyssetvalue{/sea/numeric/99p:unique_players_and_versus}{325}
\pgfkeyssetvalue{/sea/numeric/99p:courses_played}{6844}
\pgfkeyssetvalue{/sea/numeric/99p:courses_cleared}{4501.75999999791}
\pgfkeyssetvalue{/sea/numeric/99p:courses_attempted}{34643}
\pgfkeyssetvalue{/sea/numeric/99p:courses_deaths}{29540}
\pgfkeyssetvalue{/sea/numeric/99p:likes_maker}{1896}
\pgfkeyssetvalue{/sea/numeric/99p:maker_points}{7687}
\pgfkeyssetvalue{/sea/numeric/99p:easy_highscore}{1408}
\pgfkeyssetvalue{/sea/numeric/99p:normal_highscore}{547}
\pgfkeyssetvalue{/sea/numeric/99p:expert_highscore}{23}
\pgfkeyssetvalue{/sea/numeric/99p:super_expert_highscore}{4}
\pgfkeyssetvalue{/sea/numeric/99p:versus_rating}{4715}
\pgfkeyssetvalue{/sea/numeric/99p:first_clears}{215}
\pgfkeyssetvalue{/sea/numeric/99p:world_records}{268}
\pgfkeyssetvalue{/sea/numeric/99p:uploaded_levels}{100}
\pgfkeyssetvalue{/sea/numeric/99.99p:world_record}{2627.83619320001}
\pgfkeyssetvalue{/sea/numeric/99.99p:upload_time}{494.049}
\pgfkeyssetvalue{/sea/numeric/99.99p:upload_attempts}{378.027600001544}
\pgfkeyssetvalue{/sea/numeric/99.99p:num_comments}{906.055200003088}
\pgfkeyssetvalue{/sea/numeric/99.99p:timer}{500}
\pgfkeyssetvalue{/sea/numeric/99.99p:autoscroll_speed}{2}
\pgfkeyssetvalue{/sea/numeric/99.99p:clears}{15557.2208000124}
\pgfkeyssetvalue{/sea/numeric/99.99p:attempts}{142162.7940001}
\pgfkeyssetvalue{/sea/numeric/99.99p:clear_rate_p}{1}
\pgfkeyssetvalue{/sea/numeric/99.99p:likes}{4590.02760000154}
\pgfkeyssetvalue{/sea/numeric/99.99p:boos}{576}
\pgfkeyssetvalue{/sea/numeric/99.99p:unique_players_and_versus}{18171.1104000062}
\pgfkeyssetvalue{/sea/numeric/99.99p:courses_played}{63356}
\pgfkeyssetvalue{/sea/numeric/99.99p:courses_cleared}{57813}
\pgfkeyssetvalue{/sea/numeric/99.99p:courses_attempted}{452109}
\pgfkeyssetvalue{/sea/numeric/99.99p:courses_deaths}{422060}
\pgfkeyssetvalue{/sea/numeric/99.99p:likes_maker}{241521}
\pgfkeyssetvalue{/sea/numeric/99.99p:maker_points}{22633}
\pgfkeyssetvalue{/sea/numeric/99.99p:easy_highscore}{30264}
\pgfkeyssetvalue{/sea/numeric/99.99p:normal_highscore}{16501}
\pgfkeyssetvalue{/sea/numeric/99.99p:expert_highscore}{5700}
\pgfkeyssetvalue{/sea/numeric/99.99p:super_expert_highscore}{291}
\pgfkeyssetvalue{/sea/numeric/99.99p:versus_rating}{7004}
\pgfkeyssetvalue{/sea/numeric/99.99p:first_clears}{7803}
\pgfkeyssetvalue{/sea/numeric/99.99p:world_records}{10674}
\pgfkeyssetvalue{/sea/numeric/99.99p:uploaded_levels}{100}
\pgfkeyssetvalue{/sea/numeric/max:world_record}{5999.999}
\pgfkeyssetvalue{/sea/numeric/max:upload_time}{499.987}
\pgfkeyssetvalue{/sea/numeric/max:upload_attempts}{5983}
\pgfkeyssetvalue{/sea/numeric/max:num_comments}{120515}
\pgfkeyssetvalue{/sea/numeric/max:timer}{500}
\pgfkeyssetvalue{/sea/numeric/max:autoscroll_speed}{2}
\pgfkeyssetvalue{/sea/numeric/max:clears}{1804430}
\pgfkeyssetvalue{/sea/numeric/max:attempts}{67895905}
\pgfkeyssetvalue{/sea/numeric/max:clear_rate_p}{1}
\pgfkeyssetvalue{/sea/numeric/max:likes}{564890}
\pgfkeyssetvalue{/sea/numeric/max:boos}{37886}
\pgfkeyssetvalue{/sea/numeric/max:unique_players_and_versus}{1302862}
\pgfkeyssetvalue{/sea/numeric/max:courses_played}{549016}
\pgfkeyssetvalue{/sea/numeric/max:courses_cleared}{513124}
\pgfkeyssetvalue{/sea/numeric/max:courses_attempted}{17110430}
\pgfkeyssetvalue{/sea/numeric/max:courses_deaths}{17095589}
\pgfkeyssetvalue{/sea/numeric/max:likes_maker}{1278573}
\pgfkeyssetvalue{/sea/numeric/max:maker_points}{29100}
\pgfkeyssetvalue{/sea/numeric/max:easy_highscore}{320500}
\pgfkeyssetvalue{/sea/numeric/max:normal_highscore}{109304}
\pgfkeyssetvalue{/sea/numeric/max:expert_highscore}{77777}
\pgfkeyssetvalue{/sea/numeric/max:super_expert_highscore}{20000}
\pgfkeyssetvalue{/sea/numeric/max:versus_rating}{8000}
\pgfkeyssetvalue{/sea/numeric/max:first_clears}{67102}
\pgfkeyssetvalue{/sea/numeric/max:world_records}{105379}
\pgfkeyssetvalue{/sea/numeric/max:uploaded_levels}{100}
\pgfkeyssetvalue{/sea/factor/difficulty_nameEasy:Count}{8710121}
\pgfkeyssetvalue{/sea/factor/difficulty_nameEasy:Percentage}{32.7328486107992}
\pgfkeyssetvalue{/sea/factor/difficulty_nameNormal:Count}{11744359}
\pgfkeyssetvalue{/sea/factor/difficulty_nameNormal:Percentage}{44.1355895260098}
\pgfkeyssetvalue{/sea/factor/difficulty_nameExpert:Count}{4150458}
\pgfkeyssetvalue{/sea/factor/difficulty_nameExpert:Percentage}{15.5975230860146}
\pgfkeyssetvalue{/sea/factor/difficulty_nameSuper expert:Count}{2004787}
\pgfkeyssetvalue{/sea/factor/difficulty_nameSuper expert:Percentage}{7.53403877717639}
\pgfkeyssetvalue{/sea/factor/gamestyle_nameSMB1:Count}{3739380}
\pgfkeyssetvalue{/sea/factor/gamestyle_nameSMB1:Percentage}{14.0526818672497}
\pgfkeyssetvalue{/sea/factor/gamestyle_nameSMB3:Count}{2039702}
\pgfkeyssetvalue{/sea/factor/gamestyle_nameSMB3:Percentage}{7.66525020457746}
\pgfkeyssetvalue{/sea/factor/gamestyle_nameSMW:Count}{4572845}
\pgfkeyssetvalue{/sea/factor/gamestyle_nameSMW:Percentage}{17.1848638044925}
\pgfkeyssetvalue{/sea/factor/gamestyle_nameNSMBU:Count}{8750385}
\pgfkeyssetvalue{/sea/factor/gamestyle_nameNSMBU:Percentage}{32.8841617115547}
\pgfkeyssetvalue{/sea/factor/gamestyle_nameSM3DW:Count}{7507413}
\pgfkeyssetvalue{/sea/factor/gamestyle_nameSM3DW:Percentage}{28.2130424121256}
\pgfkeyssetvalue{/sea/factor/theme_nameAirship:Count}{1647068}
\pgfkeyssetvalue{/sea/factor/theme_nameAirship:Percentage}{6.18972199073835}
\pgfkeyssetvalue{/sea/factor/theme_nameCastle:Count}{3978403}
\pgfkeyssetvalue{/sea/factor/theme_nameCastle:Percentage}{14.9509361708924}
\pgfkeyssetvalue{/sea/factor/theme_nameDesert:Count}{1770880}
\pgfkeyssetvalue{/sea/factor/theme_nameDesert:Percentage}{6.65501052716629}
\pgfkeyssetvalue{/sea/factor/theme_nameForest:Count}{2188222}
\pgfkeyssetvalue{/sea/factor/theme_nameForest:Percentage}{8.2233920117551}
\pgfkeyssetvalue{/sea/factor/theme_nameGhost house:Count}{1357902}
\pgfkeyssetvalue{/sea/factor/theme_nameGhost house:Percentage}{5.1030290617434}
\pgfkeyssetvalue{/sea/factor/theme_nameOverworld:Count}{8352189}
\pgfkeyssetvalue{/sea/factor/theme_nameOverworld:Percentage}{31.3877313651306}
\pgfkeyssetvalue{/sea/factor/theme_nameSky:Count}{2610614}
\pgfkeyssetvalue{/sea/factor/theme_nameSky:Percentage}{9.81075152035581}
\pgfkeyssetvalue{/sea/factor/theme_nameSnow:Count}{2317182}
\pgfkeyssetvalue{/sea/factor/theme_nameSnow:Percentage}{8.70802685860151}
\pgfkeyssetvalue{/sea/factor/theme_nameUnderground:Count}{1846678}
\pgfkeyssetvalue{/sea/factor/theme_nameUnderground:Percentage}{6.93986127252349}
\pgfkeyssetvalue{/sea/factor/theme_nameUnderwater:Count}{540587}
\pgfkeyssetvalue{/sea/factor/theme_nameUnderwater:Percentage}{2.03153922109304}
\pgfkeyssetvalue{/sea/factor/game_versionV1.0.0:Count}{72152}
\pgfkeyssetvalue{/sea/factor/game_versionV1.0.0:Percentage}{0.271148987823061}
\pgfkeyssetvalue{/sea/factor/game_versionV1.0.1:Count}{6308783}
\pgfkeyssetvalue{/sea/factor/game_versionV1.0.1:Percentage}{23.7085614375947}
\pgfkeyssetvalue{/sea/factor/game_versionV1.1.0:Count}{1253861}
\pgfkeyssetvalue{/sea/factor/game_versionV1.1.0:Percentage}{4.71204042882818}
\pgfkeyssetvalue{/sea/factor/game_versionV2.0.0:Count}{3977634}
\pgfkeyssetvalue{/sea/factor/game_versionV2.0.0:Percentage}{14.9480462500082}
\pgfkeyssetvalue{/sea/factor/game_versionV3.0.0:Count}{3825551}
\pgfkeyssetvalue{/sea/factor/game_versionV3.0.0:Percentage}{14.3765146013347}
\pgfkeyssetvalue{/sea/factor/game_versionV3.0.1:Count}{11171744}
\pgfkeyssetvalue{/sea/factor/game_versionV3.0.1:Percentage}{41.9836882944112}
\pgfkeyssetvalue{/sea/coefs.both.user/(Intercept)/fml.all.both}{-0.290295313656599}
\pgfkeyssetvalue{/sea/coefs.both.user/difficulty_nameNormal/fml.all.both}{-0.540833733127913}
\pgfkeyssetvalue{/sea/coefs.both.user/difficulty_nameExpert/fml.all.both}{-0.841365306088128}
\pgfkeyssetvalue{/sea/coefs.both.user/difficulty_nameSuper expert/fml.all.both}{-0.976606651955006}
\pgfkeyssetvalue{/sea/coefs.both.user/upload_attempts/fml.all.both}{-0.018743900242282}
\pgfkeyssetvalue{/sea/coefs.both.user/clears/fml.all.both}{0.00471895761659158}
\pgfkeyssetvalue{/sea/coefs.both.user/attempts/fml.all.both}{-0.0044446881921083}
\pgfkeyssetvalue{/sea/coefs.both.user/likes/fml.all.both}{-0.00124465871355162}
\pgfkeyssetvalue{/sea/coefs.both.user/boos/fml.all.both}{-0.00206799699825877}
\pgfkeyssetvalue{/sea/coefs.both.user/unique_players_and_versus/fml.all.both}{0.000479176646489332}
\pgfkeyssetvalue{/sea/coefs.both.user/world_record/fml.all.both}{-0.0029628931257164}
\pgfkeyssetvalue{/sea/coefs.both.user/upload_time/fml.all.both}{-0.000407776441156638}
\pgfkeyssetvalue{/sea/coefs.both.user/num_comments/fml.all.both}{-0.0030938992788645}
\pgfkeyssetvalue{/sea/coefs.both.user/timer/fml.all.both}{0.00021496282020439}
\pgfkeyssetvalue{/sea/coefs.both.user/autoscroll_speed/fml.all.both}{0.0234437863162527}
\pgfkeyssetvalue{/sea/coefs.both.user/gamestyle_nameSMB3/fml.all.both}{-0.0157857657648561}
\pgfkeyssetvalue{/sea/coefs.both.user/gamestyle_nameSMW/fml.all.both}{-0.0236859449943184}
\pgfkeyssetvalue{/sea/coefs.both.user/gamestyle_nameNSMBU/fml.all.both}{-0.0246897205861502}
\pgfkeyssetvalue{/sea/coefs.both.user/gamestyle_nameSM3DW/fml.all.both}{0.0256482326404157}
\pgfkeyssetvalue{/sea/coefs.both.user/theme_nameCastle/fml.all.both}{-0.00710434096975077}
\pgfkeyssetvalue{/sea/coefs.both.user/theme_nameDesert/fml.all.both}{0.0152387128371081}
\pgfkeyssetvalue{/sea/coefs.both.user/theme_nameForest/fml.all.both}{0.0324368612828569}
\pgfkeyssetvalue{/sea/coefs.both.user/theme_nameGhost house/fml.all.both}{0.0211766055310261}
\pgfkeyssetvalue{/sea/coefs.both.user/theme_nameOverworld/fml.all.both}{0.0436967927125345}
\pgfkeyssetvalue{/sea/coefs.both.user/theme_nameSky/fml.all.both}{0.0307906941049028}
\pgfkeyssetvalue{/sea/coefs.both.user/theme_nameSnow/fml.all.both}{0.0332330762549315}
\pgfkeyssetvalue{/sea/coefs.both.user/theme_nameUnderground/fml.all.both}{0.0317361758791437}
\pgfkeyssetvalue{/sea/coefs.both.user/theme_nameUnderwater/fml.all.both}{0.0979670652839371}
\pgfkeyssetvalue{/sea/coefs.both.user/game_versionV1.0.1/fml.all.both}{0.0521051619043287}
\pgfkeyssetvalue{/sea/coefs.both.user/game_versionV1.1.0/fml.all.both}{0.0224892881011931}
\pgfkeyssetvalue{/sea/coefs.both.user/game_versionV2.0.0/fml.all.both}{0.00497806872480644}
\pgfkeyssetvalue{/sea/coefs.both.user/game_versionV3.0.0/fml.all.both}{-0.0149880610381877}
\pgfkeyssetvalue{/sea/coefs.both.user/game_versionV3.0.1/fml.all.both}{-0.0112616499152139}
\pgfkeyssetvalue{/sea/coefs.both.user/(Intercept)/fml.user.all}{-0.289423253172967}
\pgfkeyssetvalue{/sea/coefs.both.user/difficulty_nameNormal/fml.user.all}{-0.53899225017965}
\pgfkeyssetvalue{/sea/coefs.both.user/difficulty_nameExpert/fml.user.all}{-0.840483240044587}
\pgfkeyssetvalue{/sea/coefs.both.user/difficulty_nameSuper expert/fml.user.all}{-0.977017269422785}
\pgfkeyssetvalue{/sea/coefs.both.user/upload_attempts/fml.user.all}{-0.0172500086751786}
\pgfkeyssetvalue{/sea/coefs.both.user/clears/fml.user.all}{0.00470512061074135}
\pgfkeyssetvalue{/sea/coefs.both.user/attempts/fml.user.all}{-0.0043972198349953}
\pgfkeyssetvalue{/sea/coefs.both.user/likes/fml.user.all}{-0.000223454762014352}
\pgfkeyssetvalue{/sea/coefs.both.user/boos/fml.user.all}{0.00141584778367454}
\pgfkeyssetvalue{/sea/coefs.both.user/world_record/fml.user.all}{-0.00320447901056031}
\pgfkeyssetvalue{/sea/coefs.both.user/num_comments/fml.user.all}{-0.00162398877484959}
\pgfkeyssetvalue{/sea/coefs.both.user/autoscroll_speed/fml.user.all}{0.0145812161707053}
\pgfkeyssetvalue{/sea/coefs.both.user/gamestyle_nameSMB3/fml.user.all}{-0.0164493482927988}
\pgfkeyssetvalue{/sea/coefs.both.user/gamestyle_nameSMW/fml.user.all}{-0.0207627515584087}
\pgfkeyssetvalue{/sea/coefs.both.user/gamestyle_nameNSMBU/fml.user.all}{-0.0233503077582833}
\pgfkeyssetvalue{/sea/coefs.both.user/gamestyle_nameSM3DW/fml.user.all}{0.0281192471951481}
\pgfkeyssetvalue{/sea/coefs.both.user/theme_nameCastle/fml.user.all}{-0.00923907367944665}
\pgfkeyssetvalue{/sea/coefs.both.user/theme_nameDesert/fml.user.all}{0.0139118290403921}
\pgfkeyssetvalue{/sea/coefs.both.user/theme_nameForest/fml.user.all}{0.0298820595645692}
\pgfkeyssetvalue{/sea/coefs.both.user/theme_nameGhost house/fml.user.all}{0.0168181788745985}
\pgfkeyssetvalue{/sea/coefs.both.user/theme_nameOverworld/fml.user.all}{0.0388812284335691}
\pgfkeyssetvalue{/sea/coefs.both.user/theme_nameSky/fml.user.all}{0.0233705137738354}
\pgfkeyssetvalue{/sea/coefs.both.user/theme_nameSnow/fml.user.all}{0.0295057517143213}
\pgfkeyssetvalue{/sea/coefs.both.user/theme_nameUnderground/fml.user.all}{0.0276349068672619}
\pgfkeyssetvalue{/sea/coefs.both.user/theme_nameUnderwater/fml.user.all}{0.0986482328166121}
\pgfkeyssetvalue{/sea/coefs.both.user/game_versionV1.0.1/fml.user.all}{0.0501477849181335}
\pgfkeyssetvalue{/sea/coefs.both.user/game_versionV1.1.0/fml.user.all}{0.0082294545336119}
\pgfkeyssetvalue{/sea/coefs.both.user/game_versionV2.0.0/fml.user.all}{-0.00452822958146437}
\pgfkeyssetvalue{/sea/coefs.both.user/game_versionV3.0.0/fml.user.all}{-0.0184803780491776}
\pgfkeyssetvalue{/sea/coefs.both.user/game_versionV3.0.1/fml.user.all}{-0.0154722811569377}
\pgfkeyssetvalue{/sea/coefs.both.user/courses_played/fml.user.all}{6.27850852885636e-06}
\pgfkeyssetvalue{/sea/coefs.both.user/courses_cleared/fml.user.all}{-5.32882748893737e-06}
\pgfkeyssetvalue{/sea/coefs.both.user/courses_attempted/fml.user.all}{2.45344370508604e-06}
\pgfkeyssetvalue{/sea/coefs.both.user/courses_deaths/fml.user.all}{-2.38719467737791e-06}
\pgfkeyssetvalue{/sea/coefs.both.user/maker_points/fml.user.all}{4.68649484717254e-05}
\pgfkeyssetvalue{/sea/coefs.both.user/easy_highscore/fml.user.all}{-3.00485995918809e-06}
\pgfkeyssetvalue{/sea/coefs.both.user/normal_highscore/fml.user.all}{-1.81490359119074e-06}
\pgfkeyssetvalue{/sea/coefs.both.user/expert_highscore/fml.user.all}{-1.68423898204706e-05}
\pgfkeyssetvalue{/sea/coefs.both.user/super_expert_highscore/fml.user.all}{7.45848771990243e-05}
\pgfkeyssetvalue{/sea/coefs.both.user/versus_rating/fml.user.all}{-3.02737005131171e-06}
\pgfkeyssetvalue{/sea/coefs.both.user/first_clears/fml.user.all}{-2.18454907330301e-06}
\pgfkeyssetvalue{/sea/coefs.both.user/world_records/fml.user.all}{-1.78756636828314e-05}
\pgfkeyssetvalue{/sea/coefs.both.user/uploaded_levels/fml.user.all}{-0.000533268348545168}
\pgfkeyssetvalue{/sea/coefs.both.user/comments_enabledTRUE/fml.user.all}{0.00177886912002223}
\pgfkeyssetvalue{/sea/coefs.both.user/regionAmericas/fml.user.all}{-0.00943453608831357}
\pgfkeyssetvalue{/sea/coefs.both.user/regionEurope/fml.user.all}{-0.0167926360173115}
\pgfkeyssetvalue{/sea/coefs.both.user/regionOther/fml.user.all}{-0.00382349490939504}
\pgfkeyssetvalue{/sea/coefs.both.user/likes_maker/fml.user.all}{-2.98733276593577e-06}
\pgfkeyssetvalue{/sea/coefs.df/difficulty_nameNormal/fml.all.attempts}{-0.57192416021069}
\pgfkeyssetvalue{/sea/coefs.df/difficulty_nameExpert/fml.all.attempts}{-0.864410919617049}
\pgfkeyssetvalue{/sea/coefs.df/difficulty_nameSuper expert/fml.all.attempts}{-0.976809259160799}
\pgfkeyssetvalue{/sea/coefs.df/upload_attempts/fml.all.attempts}{-0.0223605449202414}
\pgfkeyssetvalue{/sea/coefs.df/attempts/fml.all.attempts}{-0.00111273531513889}
\pgfkeyssetvalue{/sea/coefs.df/likes/fml.all.attempts}{-0.00172475276192985}
\pgfkeyssetvalue{/sea/coefs.df/boos/fml.all.attempts}{-0.0135800987651035}
\pgfkeyssetvalue{/sea/coefs.df/unique_players_and_versus/fml.all.attempts}{0.0014620582457392}
\pgfkeyssetvalue{/sea/coefs.df/world_record/fml.all.attempts}{-0.00286554759797131}
\pgfkeyssetvalue{/sea/coefs.df/upload_time/fml.all.attempts}{-0.00078134339789504}
\pgfkeyssetvalue{/sea/coefs.df/num_comments/fml.all.attempts}{0.000963023453203649}
\pgfkeyssetvalue{/sea/coefs.df/timer/fml.all.attempts}{0.000248645157757466}
\pgfkeyssetvalue{/sea/coefs.df/autoscroll_speed/fml.all.attempts}{0.0237654178156304}
\pgfkeyssetvalue{/sea/coefs.df/gamestyle_nameSMB3/fml.all.attempts}{-0.0189328524448932}
\pgfkeyssetvalue{/sea/coefs.df/gamestyle_nameSMW/fml.all.attempts}{-0.0275090737918308}
\pgfkeyssetvalue{/sea/coefs.df/gamestyle_nameNSMBU/fml.all.attempts}{-0.0236899266052563}
\pgfkeyssetvalue{/sea/coefs.df/gamestyle_nameSM3DW/fml.all.attempts}{0.0355721952355501}
\pgfkeyssetvalue{/sea/coefs.df/theme_nameCastle/fml.all.attempts}{-0.00855065745501915}
\pgfkeyssetvalue{/sea/coefs.df/theme_nameDesert/fml.all.attempts}{0.0114106699569416}
\pgfkeyssetvalue{/sea/coefs.df/theme_nameForest/fml.all.attempts}{0.0340031064704864}
\pgfkeyssetvalue{/sea/coefs.df/theme_nameGhost house/fml.all.attempts}{0.0310998634608146}
\pgfkeyssetvalue{/sea/coefs.df/theme_nameOverworld/fml.all.attempts}{0.0438851314070066}
\pgfkeyssetvalue{/sea/coefs.df/theme_nameSky/fml.all.attempts}{0.0291483198057378}
\pgfkeyssetvalue{/sea/coefs.df/theme_nameSnow/fml.all.attempts}{0.0330936116388918}
\pgfkeyssetvalue{/sea/coefs.df/theme_nameUnderground/fml.all.attempts}{0.0362669367687585}
\pgfkeyssetvalue{/sea/coefs.df/theme_nameUnderwater/fml.all.attempts}{0.122417813758938}
\pgfkeyssetvalue{/sea/coefs.df/game_versionV1.0.1/fml.all.attempts}{0.0248643446505741}
\pgfkeyssetvalue{/sea/coefs.df/game_versionV1.1.0/fml.all.attempts}{0.0156663528706402}
\pgfkeyssetvalue{/sea/coefs.df/game_versionV2.0.0/fml.all.attempts}{0.00648286883000582}
\pgfkeyssetvalue{/sea/coefs.df/game_versionV3.0.0/fml.all.attempts}{-0.00640885394855772}
\pgfkeyssetvalue{/sea/coefs.df/game_versionV3.0.1/fml.all.attempts}{0.0103961778390094}
\pgfkeyssetvalue{/sea/coefs.df/difficulty_nameNormal/fml.all.clears}{-0.585440475495142}
\pgfkeyssetvalue{/sea/coefs.df/difficulty_nameExpert/fml.all.clears}{-0.877229204887441}
\pgfkeyssetvalue{/sea/coefs.df/difficulty_nameSuper expert/fml.all.clears}{-0.978478308068913}
\pgfkeyssetvalue{/sea/coefs.df/upload_attempts/fml.all.clears}{-0.0226884445323375}
\pgfkeyssetvalue{/sea/coefs.df/clears/fml.all.clears}{5.67274284235531e-06}
\pgfkeyssetvalue{/sea/coefs.df/likes/fml.all.clears}{-8.5652106083689e-05}
\pgfkeyssetvalue{/sea/coefs.df/boos/fml.all.clears}{-0.000176447664158808}
\pgfkeyssetvalue{/sea/coefs.df/unique_players_and_versus/fml.all.clears}{2.20754363544629e-05}
\pgfkeyssetvalue{/sea/coefs.df/world_record/fml.all.clears}{-0.0025216250066995}
\pgfkeyssetvalue{/sea/coefs.df/upload_time/fml.all.clears}{-0.000876226581352668}
\pgfkeyssetvalue{/sea/coefs.df/num_comments/fml.all.clears}{3.21536263037103e-05}
\pgfkeyssetvalue{/sea/coefs.df/timer/fml.all.clears}{0.000267297035997371}
\pgfkeyssetvalue{/sea/coefs.df/autoscroll_speed/fml.all.clears}{0.0261638095219949}
\pgfkeyssetvalue{/sea/coefs.df/gamestyle_nameSMB3/fml.all.clears}{-0.021825700125774}
\pgfkeyssetvalue{/sea/coefs.df/gamestyle_nameSMW/fml.all.clears}{-0.0293880550285828}
\pgfkeyssetvalue{/sea/coefs.df/gamestyle_nameNSMBU/fml.all.clears}{-0.0237992509069036}
\pgfkeyssetvalue{/sea/coefs.df/gamestyle_nameSM3DW/fml.all.clears}{0.0361061277830348}
\pgfkeyssetvalue{/sea/coefs.df/theme_nameCastle/fml.all.clears}{-0.0100234642962215}
\pgfkeyssetvalue{/sea/coefs.df/theme_nameDesert/fml.all.clears}{0.0093393414120122}
\pgfkeyssetvalue{/sea/coefs.df/theme_nameForest/fml.all.clears}{0.0345550476839549}
\pgfkeyssetvalue{/sea/coefs.df/theme_nameGhost house/fml.all.clears}{0.0344245430282033}
\pgfkeyssetvalue{/sea/coefs.df/theme_nameOverworld/fml.all.clears}{0.0387476119497487}
\pgfkeyssetvalue{/sea/coefs.df/theme_nameSky/fml.all.clears}{0.0257188871834229}
\pgfkeyssetvalue{/sea/coefs.df/theme_nameSnow/fml.all.clears}{0.0305010218132584}
\pgfkeyssetvalue{/sea/coefs.df/theme_nameUnderground/fml.all.clears}{0.0369803269779985}
\pgfkeyssetvalue{/sea/coefs.df/theme_nameUnderwater/fml.all.clears}{0.140242104102455}
\pgfkeyssetvalue{/sea/coefs.df/game_versionV1.0.1/fml.all.clears}{-0.00483571546318617}
\pgfkeyssetvalue{/sea/coefs.df/game_versionV1.1.0/fml.all.clears}{0.0061670716074218}
\pgfkeyssetvalue{/sea/coefs.df/game_versionV2.0.0/fml.all.clears}{0.00652215421121083}
\pgfkeyssetvalue{/sea/coefs.df/game_versionV3.0.0/fml.all.clears}{0.00862101856401498}
\pgfkeyssetvalue{/sea/coefs.df/game_versionV3.0.1/fml.all.clears}{0.0333627129737799}
\pgfkeyssetvalue{/sea/coefs.df/difficulty_nameNormal/fml.all}{-0.585472417768336}
\pgfkeyssetvalue{/sea/coefs.df/difficulty_nameExpert/fml.all}{-0.877247615459857}
\pgfkeyssetvalue{/sea/coefs.df/difficulty_nameSuper expert/fml.all}{-0.978485406732147}
\pgfkeyssetvalue{/sea/coefs.df/upload_attempts/fml.all}{-0.0226884221642432}
\pgfkeyssetvalue{/sea/coefs.df/likes/fml.all}{-7.48710430488186e-05}
\pgfkeyssetvalue{/sea/coefs.df/boos/fml.all}{-0.000137135627584439}
\pgfkeyssetvalue{/sea/coefs.df/unique_players_and_versus/fml.all}{2.41009237818002e-05}
\pgfkeyssetvalue{/sea/coefs.df/world_record/fml.all}{-0.00252362333504885}
\pgfkeyssetvalue{/sea/coefs.df/upload_time/fml.all}{-0.000876735141684626}
\pgfkeyssetvalue{/sea/coefs.df/num_comments/fml.all}{4.52777860853182e-05}
\pgfkeyssetvalue{/sea/coefs.df/timer/fml.all}{0.000267179369651149}
\pgfkeyssetvalue{/sea/coefs.df/autoscroll_speed/fml.all}{0.0260603780357469}
\pgfkeyssetvalue{/sea/coefs.df/gamestyle_nameSMB3/fml.all}{-0.021790509793402}
\pgfkeyssetvalue{/sea/coefs.df/gamestyle_nameSMW/fml.all}{-0.029349659520434}
\pgfkeyssetvalue{/sea/coefs.df/gamestyle_nameNSMBU/fml.all}{-0.0237670552310847}
\pgfkeyssetvalue{/sea/coefs.df/gamestyle_nameSM3DW/fml.all}{0.0361384538991556}
\pgfkeyssetvalue{/sea/coefs.df/theme_nameCastle/fml.all}{-0.0100195101488919}
\pgfkeyssetvalue{/sea/coefs.df/theme_nameDesert/fml.all}{0.00934099955315393}
\pgfkeyssetvalue{/sea/coefs.df/theme_nameForest/fml.all}{0.0345693861332028}
\pgfkeyssetvalue{/sea/coefs.df/theme_nameGhost house/fml.all}{0.0344123034710366}
\pgfkeyssetvalue{/sea/coefs.df/theme_nameOverworld/fml.all}{0.038745480094919}
\pgfkeyssetvalue{/sea/coefs.df/theme_nameSky/fml.all}{0.0257132823985571}
\pgfkeyssetvalue{/sea/coefs.df/theme_nameSnow/fml.all}{0.0304920750450994}
\pgfkeyssetvalue{/sea/coefs.df/theme_nameUnderground/fml.all}{0.0369914788041739}
\pgfkeyssetvalue{/sea/coefs.df/theme_nameUnderwater/fml.all}{0.1402577474933}
\pgfkeyssetvalue{/sea/coefs.df/game_versionV1.0.1/fml.all}{-0.00485371622130393}
\pgfkeyssetvalue{/sea/coefs.df/game_versionV1.1.0/fml.all}{0.00618158545461234}
\pgfkeyssetvalue{/sea/coefs.df/game_versionV2.0.0/fml.all}{0.00653007516339166}
\pgfkeyssetvalue{/sea/coefs.df/game_versionV3.0.0/fml.all}{0.00863794346959956}
\pgfkeyssetvalue{/sea/coefs.df/game_versionV3.0.1/fml.all}{0.0333666301452329}
\pgfkeyssetvalue{/sea/coefs.df/difficulty_nameNormal/fml.all.both}{-0.540833733127913}
\pgfkeyssetvalue{/sea/coefs.df/difficulty_nameExpert/fml.all.both}{-0.841365306088128}
\pgfkeyssetvalue{/sea/coefs.df/difficulty_nameSuper expert/fml.all.both}{-0.976606651955006}
\pgfkeyssetvalue{/sea/coefs.df/upload_attempts/fml.all.both}{-0.018743900242282}
\pgfkeyssetvalue{/sea/coefs.df/clears/fml.all.both}{0.00471895761659158}
\pgfkeyssetvalue{/sea/coefs.df/attempts/fml.all.both}{-0.0044446881921083}
\pgfkeyssetvalue{/sea/coefs.df/likes/fml.all.both}{-0.00124465871355162}
\pgfkeyssetvalue{/sea/coefs.df/boos/fml.all.both}{-0.00206799699825877}
\pgfkeyssetvalue{/sea/coefs.df/unique_players_and_versus/fml.all.both}{0.000479176646489332}
\pgfkeyssetvalue{/sea/coefs.df/world_record/fml.all.both}{-0.0029628931257164}
\pgfkeyssetvalue{/sea/coefs.df/upload_time/fml.all.both}{-0.000407776441156638}
\pgfkeyssetvalue{/sea/coefs.df/num_comments/fml.all.both}{-0.0030938992788645}
\pgfkeyssetvalue{/sea/coefs.df/timer/fml.all.both}{0.00021496282020439}
\pgfkeyssetvalue{/sea/coefs.df/autoscroll_speed/fml.all.both}{0.0234437863162527}
\pgfkeyssetvalue{/sea/coefs.df/gamestyle_nameSMB3/fml.all.both}{-0.0157857657648561}
\pgfkeyssetvalue{/sea/coefs.df/gamestyle_nameSMW/fml.all.both}{-0.0236859449943184}
\pgfkeyssetvalue{/sea/coefs.df/gamestyle_nameNSMBU/fml.all.both}{-0.0246897205861502}
\pgfkeyssetvalue{/sea/coefs.df/gamestyle_nameSM3DW/fml.all.both}{0.0256482326404157}
\pgfkeyssetvalue{/sea/coefs.df/theme_nameCastle/fml.all.both}{-0.00710434096975077}
\pgfkeyssetvalue{/sea/coefs.df/theme_nameDesert/fml.all.both}{0.0152387128371081}
\pgfkeyssetvalue{/sea/coefs.df/theme_nameForest/fml.all.both}{0.0324368612828569}
\pgfkeyssetvalue{/sea/coefs.df/theme_nameGhost house/fml.all.both}{0.0211766055310261}
\pgfkeyssetvalue{/sea/coefs.df/theme_nameOverworld/fml.all.both}{0.0436967927125345}
\pgfkeyssetvalue{/sea/coefs.df/theme_nameSky/fml.all.both}{0.0307906941049028}
\pgfkeyssetvalue{/sea/coefs.df/theme_nameSnow/fml.all.both}{0.0332330762549315}
\pgfkeyssetvalue{/sea/coefs.df/theme_nameUnderground/fml.all.both}{0.0317361758791437}
\pgfkeyssetvalue{/sea/coefs.df/theme_nameUnderwater/fml.all.both}{0.0979670652839371}
\pgfkeyssetvalue{/sea/coefs.df/game_versionV1.0.1/fml.all.both}{0.0521051619043287}
\pgfkeyssetvalue{/sea/coefs.df/game_versionV1.1.0/fml.all.both}{0.0224892881011931}
\pgfkeyssetvalue{/sea/coefs.df/game_versionV2.0.0/fml.all.both}{0.00497806872480644}
\pgfkeyssetvalue{/sea/coefs.df/game_versionV3.0.0/fml.all.both}{-0.0149880610381877}
\pgfkeyssetvalue{/sea/coefs.df/game_versionV3.0.1/fml.all.both}{-0.0112616499152139}
\pgfkeyssetvalue{/sea/average.effects/upload_attempts/fml.all.both:mean_delta}{-0.10222727652608}
\pgfkeyssetvalue{/sea/average.effects/upload_attempts/fml.all.both:mean_diff}{5.69916028800128}
\pgfkeyssetvalue{/sea/average.effects/clears/fml.all.both:mean_delta}{0.224960339146886}
\pgfkeyssetvalue{/sea/average.effects/clears/fml.all.both:mean_diff}{43.0999526516648}
\pgfkeyssetvalue{/sea/average.effects/attempts/fml.all.both:mean_delta}{-0.671088097118267}
\pgfkeyssetvalue{/sea/average.effects/attempts/fml.all.both:mean_diff}{249.622084663547}
\pgfkeyssetvalue{/sea/average.effects/likes/fml.all.both:mean_delta}{-0.0108245629006227}
\pgfkeyssetvalue{/sea/average.effects/likes/fml.all.both:mean_diff}{8.73878118316051}
\pgfkeyssetvalue{/sea/average.effects/boos/fml.all.both:mean_delta}{-0.00582270546019859}
\pgfkeyssetvalue{/sea/average.effects/boos/fml.all.both:mean_diff}{2.82093405296234}
\pgfkeyssetvalue{/sea/average.effects/unique_players_and_versus/fml.all.both:mean_delta}{0.0288339887380029}
\pgfkeyssetvalue{/sea/average.effects/unique_players_and_versus/fml.all.both:mean_diff}{59.3370345761482}
\pgfkeyssetvalue{/sea/average.effects/world_record/fml.all.both:mean_delta}{-0.120705275937001}
\pgfkeyssetvalue{/sea/average.effects/world_record/fml.all.both:mean_diff}{43.351034609338}
\pgfkeyssetvalue{/sea/average.effects/upload_time/fml.all.both:mean_delta}{-0.0209181925777576}
\pgfkeyssetvalue{/sea/average.effects/upload_time/fml.all.both:mean_diff}{51.8317516037236}
\pgfkeyssetvalue{/sea/average.effects/num_comments/fml.all.both:mean_delta}{-0.00586287082201631}
\pgfkeyssetvalue{/sea/average.effects/num_comments/fml.all.both:mean_diff}{1.8976131532365}
\pgfkeyssetvalue{/sea/average.effects/timer/fml.all.both:mean_delta}{0.0211647912653332}
\pgfkeyssetvalue{/sea/average.effects/timer/fml.all.both:mean_diff}{97.440938707344}
\pgfkeyssetvalue{/sea/average.effects/autoscroll_speed/fml.all.both:mean_delta}{0.0006277767462044}
\pgfkeyssetvalue{/sea/average.effects/autoscroll_speed/fml.all.both:mean_diff}{0.0270821350960989}
\pgfkeyssetvalue{/sea/average.effects/upload_attempts/fml.user.all:mean_delta}{-0.0944097813616092}
\pgfkeyssetvalue{/sea/average.effects/upload_attempts/fml.user.all:mean_diff}{5.69916028800128}
\pgfkeyssetvalue{/sea/average.effects/clears/fml.user.all:mean_delta}{0.224233446205329}
\pgfkeyssetvalue{/sea/average.effects/clears/fml.user.all:mean_diff}{43.0999526516648}
\pgfkeyssetvalue{/sea/average.effects/attempts/fml.user.all:mean_delta}{-0.667150075925706}
\pgfkeyssetvalue{/sea/average.effects/attempts/fml.user.all:mean_diff}{249.622084663547}
\pgfkeyssetvalue{/sea/average.effects/likes/fml.user.all:mean_delta}{-0.00195103472718716}
\pgfkeyssetvalue{/sea/average.effects/likes/fml.user.all:mean_diff}{8.73878118316051}
\pgfkeyssetvalue{/sea/average.effects/boos/fml.user.all:mean_delta}{0.00399916383486754}
\pgfkeyssetvalue{/sea/average.effects/boos/fml.user.all:mean_diff}{2.82093405296234}
\pgfkeyssetvalue{/sea/average.effects/world_record/fml.user.all:mean_delta}{-0.12989426149971}
\pgfkeyssetvalue{/sea/average.effects/world_record/fml.user.all:mean_diff}{43.351034609338}
\pgfkeyssetvalue{/sea/average.effects/num_comments/fml.user.all:mean_delta}{-0.00307945621539152}
\pgfkeyssetvalue{/sea/average.effects/num_comments/fml.user.all:mean_diff}{1.8976131532365}
\pgfkeyssetvalue{/sea/average.effects/autoscroll_speed/fml.user.all:mean_delta}{0.000392116015575095}
\pgfkeyssetvalue{/sea/average.effects/autoscroll_speed/fml.user.all:mean_diff}{0.0270821350960989}
\pgfkeyssetvalue{/sea/average.effects/courses_played/fml.user.all:mean_delta}{0.00632255085270628}
\pgfkeyssetvalue{/sea/average.effects/courses_played/fml.user.all:mean_diff}{1003.84783017433}
\pgfkeyssetvalue{/sea/average.effects/courses_cleared/fml.user.all:mean_delta}{-0.00351308085472368}
\pgfkeyssetvalue{/sea/average.effects/courses_cleared/fml.user.all:mean_diff}{660.418608874039}
\pgfkeyssetvalue{/sea/average.effects/courses_attempted/fml.user.all:mean_delta}{0.0118991828156407}
\pgfkeyssetvalue{/sea/average.effects/courses_attempted/fml.user.all:mean_diff}{4821.36951637481}
\pgfkeyssetvalue{/sea/average.effects/courses_deaths/fml.user.all:mean_delta}{-0.00970539899020273}
\pgfkeyssetvalue{/sea/average.effects/courses_deaths/fml.user.all:mean_diff}{4085.46139726807}
\pgfkeyssetvalue{/sea/average.effects/maker_points/fml.user.all:mean_delta}{0.0722437006183874}
\pgfkeyssetvalue{/sea/average.effects/maker_points/fml.user.all:mean_diff}{1488.42591819369}
\pgfkeyssetvalue{/sea/average.effects/easy_highscore/fml.user.all:mean_delta}{-0.000586149181218021}
\pgfkeyssetvalue{/sea/average.effects/easy_highscore/fml.user.all:mean_diff}{195.123952817593}
\pgfkeyssetvalue{/sea/average.effects/normal_highscore/fml.user.all:mean_delta}{-9.01575820871914e-05}
\pgfkeyssetvalue{/sea/average.effects/normal_highscore/fml.user.all:mean_diff}{49.6784320371207}
\pgfkeyssetvalue{/sea/average.effects/expert_highscore/fml.user.all:mean_delta}{-0.000154757307883724}
\pgfkeyssetvalue{/sea/average.effects/expert_highscore/fml.user.all:mean_diff}{9.1891935963507}
\pgfkeyssetvalue{/sea/average.effects/super_expert_highscore/fml.user.all:mean_delta}{4.79017446519681e-05}
\pgfkeyssetvalue{/sea/average.effects/super_expert_highscore/fml.user.all:mean_diff}{0.64225330263758}
\pgfkeyssetvalue{/sea/average.effects/versus_rating/fml.user.all:mean_delta}{-0.00396168461008828}
\pgfkeyssetvalue{/sea/average.effects/versus_rating/fml.user.all:mean_diff}{1311.21957162346}
\pgfkeyssetvalue{/sea/average.effects/first_clears/fml.user.all:mean_delta}{-6.89922776682117e-05}
\pgfkeyssetvalue{/sea/average.effects/first_clears/fml.user.all:mean_diff}{31.5829858101682}
\pgfkeyssetvalue{/sea/average.effects/world_records/fml.user.all:mean_delta}{-0.000588279049220763}
\pgfkeyssetvalue{/sea/average.effects/world_records/fml.user.all:mean_diff}{32.9188836941522}
\pgfkeyssetvalue{/sea/average.effects/uploaded_levels/fml.user.all:mean_delta}{-0.0169505715611721}
\pgfkeyssetvalue{/sea/average.effects/uploaded_levels/fml.user.all:mean_diff}{32.050126622664}
\pgfkeyssetvalue{/sea/average.effects/likes_maker/fml.user.all:mean_delta}{-0.00105721912502821}
\pgfkeyssetvalue{/sea/average.effects/likes_maker/fml.user.all:mean_diff}{354.087367655122}
\pgfkeyssetvalue{/sea/N.99.players}{267089}
\pgfkeyssetvalue{/sea/N.99.9.players}{26610}
\pgfkeyssetvalue{/sea/N.99.makers}{266120}
\pgfkeyssetvalue{/sea/N.99.9.makers}{26678}
\pgfkeyssetvalue{/sea/N.99.9.both}{12748}
\pgfkeyssetvalue{/sea/N.99.9.both.percent.players}{0.479068019541526}
\pgfkeyssetvalue{/sea/N.99.9.both.percent.makers}{0.477846915061099}
\pgfkeyssetvalue{/sea/diff.coefs/difficulty_nameNormal:fml.user.all:data_99_9_players}{0.0528866789590141}
\pgfkeyssetvalue{/sea/diff.coefs/difficulty_nameExpert:fml.user.all:data_99_9_players}{0.0790332222992949}
\pgfkeyssetvalue{/sea/diff.coefs/difficulty_nameSuper expert:fml.user.all:data_99_9_players}{0.0755996816970362}
\pgfkeyssetvalue{/sea/diff.coefs/upload_attempts:fml.user.all:data_99_9_players}{-0.000205382062725357}
\pgfkeyssetvalue{/sea/diff.coefs/clears:fml.user.all:data_99_9_players}{-0.00467674328409418}
\pgfkeyssetvalue{/sea/diff.coefs/attempts:fml.user.all:data_99_9_players}{0.00437042640730967}
\pgfkeyssetvalue{/sea/diff.coefs/likes:fml.user.all:data_99_9_players}{0.000241191979153843}
\pgfkeyssetvalue{/sea/diff.coefs/boos:fml.user.all:data_99_9_players}{-0.0013780311448095}
\pgfkeyssetvalue{/sea/diff.coefs/world_record:fml.user.all:data_99_9_players}{0.00334693467669123}
\pgfkeyssetvalue{/sea/diff.coefs/num_comments:fml.user.all:data_99_9_players}{0.00159824191071245}
\pgfkeyssetvalue{/sea/diff.coefs/autoscroll_speed:fml.user.all:data_99_9_players}{0.010449754091449}
\pgfkeyssetvalue{/sea/diff.coefs/gamestyle_nameSMB3:fml.user.all:data_99_9_players}{-0.0455412827911497}
\pgfkeyssetvalue{/sea/diff.coefs/gamestyle_nameSMW:fml.user.all:data_99_9_players}{-0.0347439615210403}
\pgfkeyssetvalue{/sea/diff.coefs/gamestyle_nameNSMBU:fml.user.all:data_99_9_players}{-0.0986516138298517}
\pgfkeyssetvalue{/sea/diff.coefs/gamestyle_nameSM3DW:fml.user.all:data_99_9_players}{-0.0660449489246109}
\pgfkeyssetvalue{/sea/diff.coefs/theme_nameCastle:fml.user.all:data_99_9_players}{0.019895235498894}
\pgfkeyssetvalue{/sea/diff.coefs/theme_nameDesert:fml.user.all:data_99_9_players}{-0.0631848279667551}
\pgfkeyssetvalue{/sea/diff.coefs/theme_nameForest:fml.user.all:data_99_9_players}{-0.0606767904590123}
\pgfkeyssetvalue{/sea/diff.coefs/theme_nameGhost house:fml.user.all:data_99_9_players}{0.00889742606732691}
\pgfkeyssetvalue{/sea/diff.coefs/theme_nameOverworld:fml.user.all:data_99_9_players}{-0.0418571053377779}
\pgfkeyssetvalue{/sea/diff.coefs/theme_nameSky:fml.user.all:data_99_9_players}{-0.000440463307426864}
\pgfkeyssetvalue{/sea/diff.coefs/theme_nameSnow:fml.user.all:data_99_9_players}{-0.0487317440741117}
\pgfkeyssetvalue{/sea/diff.coefs/theme_nameUnderground:fml.user.all:data_99_9_players}{0.000850587039265882}
\pgfkeyssetvalue{/sea/diff.coefs/theme_nameUnderwater:fml.user.all:data_99_9_players}{-0.0807247974574896}
\pgfkeyssetvalue{/sea/diff.coefs/game_versionV1.0.1:fml.user.all:data_99_9_players}{0.0393127927942853}
\pgfkeyssetvalue{/sea/diff.coefs/game_versionV1.1.0:fml.user.all:data_99_9_players}{0.0695715812968338}
\pgfkeyssetvalue{/sea/diff.coefs/game_versionV2.0.0:fml.user.all:data_99_9_players}{0.126873680389959}
\pgfkeyssetvalue{/sea/diff.coefs/game_versionV3.0.0:fml.user.all:data_99_9_players}{0.128606059522092}
\pgfkeyssetvalue{/sea/diff.coefs/game_versionV3.0.1:fml.user.all:data_99_9_players}{0.16331136563896}
\pgfkeyssetvalue{/sea/diff.coefs/courses_played:fml.user.all:data_99_9_players}{-5.24624792519468e-06}
\pgfkeyssetvalue{/sea/diff.coefs/courses_cleared:fml.user.all:data_99_9_players}{-2.65695527534859e-06}
\pgfkeyssetvalue{/sea/diff.coefs/courses_attempted:fml.user.all:data_99_9_players}{4.30026595821253e-06}
\pgfkeyssetvalue{/sea/diff.coefs/courses_deaths:fml.user.all:data_99_9_players}{-4.36162531580742e-06}
\pgfkeyssetvalue{/sea/diff.coefs/maker_points:fml.user.all:data_99_9_players}{-4.0880457869763e-05}
\pgfkeyssetvalue{/sea/diff.coefs/easy_highscore:fml.user.all:data_99_9_players}{4.32048725318435e-06}
\pgfkeyssetvalue{/sea/diff.coefs/normal_highscore:fml.user.all:data_99_9_players}{-5.78351677549271e-07}
\pgfkeyssetvalue{/sea/diff.coefs/expert_highscore:fml.user.all:data_99_9_players}{1.47295184740326e-05}
\pgfkeyssetvalue{/sea/diff.coefs/super_expert_highscore:fml.user.all:data_99_9_players}{-7.09224602257752e-05}
\pgfkeyssetvalue{/sea/diff.coefs/versus_rating:fml.user.all:data_99_9_players}{8.56985789976505e-06}
\pgfkeyssetvalue{/sea/diff.coefs/first_clears:fml.user.all:data_99_9_players}{-1.28669009624716e-06}
\pgfkeyssetvalue{/sea/diff.coefs/world_records:fml.user.all:data_99_9_players}{1.19375085009255e-05}
\pgfkeyssetvalue{/sea/diff.coefs/uploaded_levels:fml.user.all:data_99_9_players}{-0.000192331976914928}
\pgfkeyssetvalue{/sea/diff.coefs/comments_enabledTRUE:fml.user.all:data_99_9_players}{-0.00178086680238176}
\pgfkeyssetvalue{/sea/diff.coefs/regionAmericas:fml.user.all:data_99_9_players}{-0.0546440287116363}
\pgfkeyssetvalue{/sea/diff.coefs/regionEurope:fml.user.all:data_99_9_players}{-0.0448717456109428}
\pgfkeyssetvalue{/sea/diff.coefs/regionOther:fml.user.all:data_99_9_players}{-0.0609841855548167}
\pgfkeyssetvalue{/sea/diff.coefs/likes_maker:fml.user.all:data_99_9_players}{3.0722251599391e-06}
\pgfkeyssetvalue{/sea/diff.coefs/difficulty_nameNormal:fml.all.both:data_99_9_players}{0.0494301137602555}
\pgfkeyssetvalue{/sea/diff.coefs/difficulty_nameExpert:fml.all.both:data_99_9_players}{0.0639291584747207}
\pgfkeyssetvalue{/sea/diff.coefs/difficulty_nameSuper expert:fml.all.both:data_99_9_players}{0.0399496614922541}
\pgfkeyssetvalue{/sea/diff.coefs/upload_attempts:fml.all.both:data_99_9_players}{-0.0044526692462411}
\pgfkeyssetvalue{/sea/diff.coefs/clears:fml.all.both:data_99_9_players}{-0.00469442573594758}
\pgfkeyssetvalue{/sea/diff.coefs/attempts:fml.all.both:data_99_9_players}{0.00442193709685446}
\pgfkeyssetvalue{/sea/diff.coefs/likes:fml.all.both:data_99_9_players}{0.00123041122198309}
\pgfkeyssetvalue{/sea/diff.coefs/boos:fml.all.both:data_99_9_players}{0.00201105918539413}
\pgfkeyssetvalue{/sea/diff.coefs/unique_players_and_versus:fml.all.both:data_99_9_players}{-0.000468859086886209}
\pgfkeyssetvalue{/sea/diff.coefs/world_record:fml.all.both:data_99_9_players}{0.00470442697478513}
\pgfkeyssetvalue{/sea/diff.coefs/upload_time:fml.all.both:data_99_9_players}{-0.00138303952452368}
\pgfkeyssetvalue{/sea/diff.coefs/num_comments:fml.all.both:data_99_9_players}{0.00307497222819175}
\pgfkeyssetvalue{/sea/diff.coefs/timer:fml.all.both:data_99_9_players}{0.000112201882302321}
\pgfkeyssetvalue{/sea/diff.coefs/autoscroll_speed:fml.all.both:data_99_9_players}{-0.00308377716664188}
\pgfkeyssetvalue{/sea/diff.coefs/gamestyle_nameSMB3:fml.all.both:data_99_9_players}{-0.054867536097538}
\pgfkeyssetvalue{/sea/diff.coefs/gamestyle_nameSMW:fml.all.both:data_99_9_players}{-0.0389383549483248}
\pgfkeyssetvalue{/sea/diff.coefs/gamestyle_nameNSMBU:fml.all.both:data_99_9_players}{-0.103410291480613}
\pgfkeyssetvalue{/sea/diff.coefs/gamestyle_nameSM3DW:fml.all.both:data_99_9_players}{-0.0673877104199621}
\pgfkeyssetvalue{/sea/diff.coefs/theme_nameCastle:fml.all.both:data_99_9_players}{0.022857239825958}
\pgfkeyssetvalue{/sea/diff.coefs/theme_nameDesert:fml.all.both:data_99_9_players}{-0.06822691279655}
\pgfkeyssetvalue{/sea/diff.coefs/theme_nameForest:fml.all.both:data_99_9_players}{-0.0684664078443924}
\pgfkeyssetvalue{/sea/diff.coefs/theme_nameGhost house:fml.all.both:data_99_9_players}{-0.000556723748857069}
\pgfkeyssetvalue{/sea/diff.coefs/theme_nameOverworld:fml.all.both:data_99_9_players}{-0.0591474022752798}
\pgfkeyssetvalue{/sea/diff.coefs/theme_nameSky:fml.all.both:data_99_9_players}{-0.0100525026835021}
\pgfkeyssetvalue{/sea/diff.coefs/theme_nameSnow:fml.all.both:data_99_9_players}{-0.0479439487723222}
\pgfkeyssetvalue{/sea/diff.coefs/theme_nameUnderground:fml.all.both:data_99_9_players}{-0.00117929830916341}
\pgfkeyssetvalue{/sea/diff.coefs/theme_nameUnderwater:fml.all.both:data_99_9_players}{-0.087897650497252}
\pgfkeyssetvalue{/sea/diff.coefs/game_versionV1.0.1:fml.all.both:data_99_9_players}{0.0340655358629429}
\pgfkeyssetvalue{/sea/diff.coefs/game_versionV1.1.0:fml.all.both:data_99_9_players}{0.0570078962438709}
\pgfkeyssetvalue{/sea/diff.coefs/game_versionV2.0.0:fml.all.both:data_99_9_players}{0.110202803283631}
\pgfkeyssetvalue{/sea/diff.coefs/game_versionV3.0.0:fml.all.both:data_99_9_players}{0.110745565642423}
\pgfkeyssetvalue{/sea/diff.coefs/game_versionV3.0.1:fml.all.both:data_99_9_players}{0.171555942033137}
\pgfkeyssetvalue{/sea/diff.coefs/difficulty_nameNormal:fml.user.all:data_99_9_makers}{-0.0409566585900923}
\pgfkeyssetvalue{/sea/diff.coefs/difficulty_nameExpert:fml.user.all:data_99_9_makers}{-0.0176251035347488}
\pgfkeyssetvalue{/sea/diff.coefs/difficulty_nameSuper expert:fml.user.all:data_99_9_makers}{0.00904840872214796}
\pgfkeyssetvalue{/sea/diff.coefs/upload_attempts:fml.user.all:data_99_9_makers}{-0.00643772176535096}
\pgfkeyssetvalue{/sea/diff.coefs/clears:fml.user.all:data_99_9_makers}{-0.00468398358780209}
\pgfkeyssetvalue{/sea/diff.coefs/attempts:fml.user.all:data_99_9_makers}{0.00437609723822274}
\pgfkeyssetvalue{/sea/diff.coefs/likes:fml.user.all:data_99_9_makers}{0.0002404614400775}
\pgfkeyssetvalue{/sea/diff.coefs/boos:fml.user.all:data_99_9_makers}{-0.00131836691873843}
\pgfkeyssetvalue{/sea/diff.coefs/world_record:fml.user.all:data_99_9_makers}{0.00296945406310878}
\pgfkeyssetvalue{/sea/diff.coefs/num_comments:fml.user.all:data_99_9_makers}{0.00160398617822577}
\pgfkeyssetvalue{/sea/diff.coefs/autoscroll_speed:fml.user.all:data_99_9_makers}{0.00919612727101193}
\pgfkeyssetvalue{/sea/diff.coefs/gamestyle_nameSMB3:fml.user.all:data_99_9_makers}{-0.0886741799444913}
\pgfkeyssetvalue{/sea/diff.coefs/gamestyle_nameSMW:fml.user.all:data_99_9_makers}{-0.0894073192792681}
\pgfkeyssetvalue{/sea/diff.coefs/gamestyle_nameNSMBU:fml.user.all:data_99_9_makers}{-0.122033562928283}
\pgfkeyssetvalue{/sea/diff.coefs/gamestyle_nameSM3DW:fml.user.all:data_99_9_makers}{-0.0786751824721216}
\pgfkeyssetvalue{/sea/diff.coefs/theme_nameCastle:fml.user.all:data_99_9_makers}{0.0516119223701673}
\pgfkeyssetvalue{/sea/diff.coefs/theme_nameDesert:fml.user.all:data_99_9_makers}{0.00347548855052393}
\pgfkeyssetvalue{/sea/diff.coefs/theme_nameForest:fml.user.all:data_99_9_makers}{-0.00236022447927553}
\pgfkeyssetvalue{/sea/diff.coefs/theme_nameGhost house:fml.user.all:data_99_9_makers}{0.0459160044360305}
\pgfkeyssetvalue{/sea/diff.coefs/theme_nameOverworld:fml.user.all:data_99_9_makers}{0.0451789367191036}
\pgfkeyssetvalue{/sea/diff.coefs/theme_nameSky:fml.user.all:data_99_9_makers}{0.0429560864141378}
\pgfkeyssetvalue{/sea/diff.coefs/theme_nameSnow:fml.user.all:data_99_9_makers}{0.00422287568158652}
\pgfkeyssetvalue{/sea/diff.coefs/theme_nameUnderground:fml.user.all:data_99_9_makers}{0.0615572498569661}
\pgfkeyssetvalue{/sea/diff.coefs/theme_nameUnderwater:fml.user.all:data_99_9_makers}{-0.0554172488438824}
\pgfkeyssetvalue{/sea/diff.coefs/game_versionV1.0.1:fml.user.all:data_99_9_makers}{0.0812549205707349}
\pgfkeyssetvalue{/sea/diff.coefs/game_versionV1.1.0:fml.user.all:data_99_9_makers}{0.11535690216344}
\pgfkeyssetvalue{/sea/diff.coefs/game_versionV2.0.0:fml.user.all:data_99_9_makers}{0.15560255084332}
\pgfkeyssetvalue{/sea/diff.coefs/game_versionV3.0.0:fml.user.all:data_99_9_makers}{0.164839540688819}
\pgfkeyssetvalue{/sea/diff.coefs/game_versionV3.0.1:fml.user.all:data_99_9_makers}{0.184038271248051}
\pgfkeyssetvalue{/sea/diff.coefs/courses_played:fml.user.all:data_99_9_makers}{-6.43741242456475e-06}
\pgfkeyssetvalue{/sea/diff.coefs/courses_cleared:fml.user.all:data_99_9_makers}{-4.45107095248254e-06}
\pgfkeyssetvalue{/sea/diff.coefs/courses_attempted:fml.user.all:data_99_9_makers}{5.17236120001208e-06}
\pgfkeyssetvalue{/sea/diff.coefs/courses_deaths:fml.user.all:data_99_9_makers}{-5.40943624216528e-06}
\pgfkeyssetvalue{/sea/diff.coefs/maker_points:fml.user.all:data_99_9_makers}{-2.75173517489957e-05}
\pgfkeyssetvalue{/sea/diff.coefs/easy_highscore:fml.user.all:data_99_9_makers}{7.9917895438042e-06}
\pgfkeyssetvalue{/sea/diff.coefs/normal_highscore:fml.user.all:data_99_9_makers}{2.40492973624384e-06}
\pgfkeyssetvalue{/sea/diff.coefs/expert_highscore:fml.user.all:data_99_9_makers}{1.52251972700412e-05}
\pgfkeyssetvalue{/sea/diff.coefs/super_expert_highscore:fml.user.all:data_99_9_makers}{-6.10824674689425e-05}
\pgfkeyssetvalue{/sea/diff.coefs/versus_rating:fml.user.all:data_99_9_makers}{6.09486659675085e-06}
\pgfkeyssetvalue{/sea/diff.coefs/first_clears:fml.user.all:data_99_9_makers}{-2.1107298376899e-06}
\pgfkeyssetvalue{/sea/diff.coefs/world_records:fml.user.all:data_99_9_makers}{1.41616473856576e-05}
\pgfkeyssetvalue{/sea/diff.coefs/uploaded_levels:fml.user.all:data_99_9_makers}{0.00019250157567885}
\pgfkeyssetvalue{/sea/diff.coefs/comments_enabledTRUE:fml.user.all:data_99_9_makers}{-0.0351276646823313}
\pgfkeyssetvalue{/sea/diff.coefs/regionAmericas:fml.user.all:data_99_9_makers}{-0.0471200611709415}
\pgfkeyssetvalue{/sea/diff.coefs/regionEurope:fml.user.all:data_99_9_makers}{-0.0520860126485244}
\pgfkeyssetvalue{/sea/diff.coefs/regionOther:fml.user.all:data_99_9_makers}{-0.0977833851334055}
\pgfkeyssetvalue{/sea/diff.coefs/likes_maker:fml.user.all:data_99_9_makers}{2.91997508983233e-06}
\pgfkeyssetvalue{/sea/diff.coefs/difficulty_nameNormal:fml.all.both:data_99_9_makers}{-0.0404375058845632}
\pgfkeyssetvalue{/sea/diff.coefs/difficulty_nameExpert:fml.all.both:data_99_9_makers}{-0.0188165059583724}
\pgfkeyssetvalue{/sea/diff.coefs/difficulty_nameSuper expert:fml.all.both:data_99_9_makers}{0.0087064440891601}
\pgfkeyssetvalue{/sea/diff.coefs/upload_attempts:fml.all.both:data_99_9_makers}{-0.011444212200566}
\pgfkeyssetvalue{/sea/diff.coefs/clears:fml.all.both:data_99_9_makers}{-0.00470184550982422}
\pgfkeyssetvalue{/sea/diff.coefs/attempts:fml.all.both:data_99_9_makers}{0.00442809743030037}
\pgfkeyssetvalue{/sea/diff.coefs/likes:fml.all.both:data_99_9_makers}{0.00122255579178077}
\pgfkeyssetvalue{/sea/diff.coefs/boos:fml.all.both:data_99_9_makers}{0.0020573334870736}
\pgfkeyssetvalue{/sea/diff.coefs/unique_players_and_versus:fml.all.both:data_99_9_makers}{-0.000467204587460746}
\pgfkeyssetvalue{/sea/diff.coefs/world_record:fml.all.both:data_99_9_makers}{0.00318585737188126}
\pgfkeyssetvalue{/sea/diff.coefs/upload_time:fml.all.both:data_99_9_makers}{-0.000754417102205251}
\pgfkeyssetvalue{/sea/diff.coefs/num_comments:fml.all.both:data_99_9_makers}{0.00308370376718881}
\pgfkeyssetvalue{/sea/diff.coefs/timer:fml.all.both:data_99_9_makers}{0.000301857094757274}
\pgfkeyssetvalue{/sea/diff.coefs/autoscroll_speed:fml.all.both:data_99_9_makers}{-0.0112085103432775}
\pgfkeyssetvalue{/sea/diff.coefs/gamestyle_nameSMB3:fml.all.both:data_99_9_makers}{-0.100170729615353}
\pgfkeyssetvalue{/sea/diff.coefs/gamestyle_nameSMW:fml.all.both:data_99_9_makers}{-0.0858395847210125}
\pgfkeyssetvalue{/sea/diff.coefs/gamestyle_nameNSMBU:fml.all.both:data_99_9_makers}{-0.11760922416708}
\pgfkeyssetvalue{/sea/diff.coefs/gamestyle_nameSM3DW:fml.all.both:data_99_9_makers}{-0.0769065086703223}
\pgfkeyssetvalue{/sea/diff.coefs/theme_nameCastle:fml.all.both:data_99_9_makers}{0.0436459915922939}
\pgfkeyssetvalue{/sea/diff.coefs/theme_nameDesert:fml.all.both:data_99_9_makers}{-0.0112606676841145}
\pgfkeyssetvalue{/sea/diff.coefs/theme_nameForest:fml.all.both:data_99_9_makers}{-0.0223157991744913}
\pgfkeyssetvalue{/sea/diff.coefs/theme_nameGhost house:fml.all.both:data_99_9_makers}{0.0224041719590411}
\pgfkeyssetvalue{/sea/diff.coefs/theme_nameOverworld:fml.all.both:data_99_9_makers}{0.026052252408912}
\pgfkeyssetvalue{/sea/diff.coefs/theme_nameSky:fml.all.both:data_99_9_makers}{0.0281325460933466}
\pgfkeyssetvalue{/sea/diff.coefs/theme_nameSnow:fml.all.both:data_99_9_makers}{0.00682166280507146}
\pgfkeyssetvalue{/sea/diff.coefs/theme_nameUnderground:fml.all.both:data_99_9_makers}{0.0629883042121917}
\pgfkeyssetvalue{/sea/diff.coefs/theme_nameUnderwater:fml.all.both:data_99_9_makers}{-0.060177358676502}
\pgfkeyssetvalue{/sea/diff.coefs/game_versionV1.0.1:fml.all.both:data_99_9_makers}{0.134121030276683}
\pgfkeyssetvalue{/sea/diff.coefs/game_versionV1.1.0:fml.all.both:data_99_9_makers}{0.133413003071847}
\pgfkeyssetvalue{/sea/diff.coefs/game_versionV2.0.0:fml.all.both:data_99_9_makers}{0.173387785122898}
\pgfkeyssetvalue{/sea/diff.coefs/game_versionV3.0.0:fml.all.both:data_99_9_makers}{0.184897629311853}
\pgfkeyssetvalue{/sea/diff.coefs/game_versionV3.0.1:fml.all.both:data_99_9_makers}{0.225088729278277}
\pgfkeyssetvalue{/sea/insignificant.vars/data_99_9_makers:fml.all.both:N_vars}{11}
\pgfkeyssetvalue{/sea/insignificant.vars/data_99_9_makers:fml.user.all:N_vars}{26}
\pgfkeyssetvalue{/sea/insignificant.vars/data_99_9_players:fml.all.both:N_vars}{13}
\pgfkeyssetvalue{/sea/insignificant.vars/data_99_9_players:fml.user.all:N_vars}{25}
\pgfkeyssetvalue{/sea/N.fml.causal.variables}{4}
\pgfkeyssetvalue{/sea/coefs.causal/(Intercept)/fml.causal}{-0.506321105127101}
\pgfkeyssetvalue{/sea/coefs.causal/gamestyle_nameSMB3/fml.causal}{-0.0681488942702818}
\pgfkeyssetvalue{/sea/coefs.causal/gamestyle_nameSMW/fml.causal}{-0.117399930025597}
\pgfkeyssetvalue{/sea/coefs.causal/gamestyle_nameNSMBU/fml.causal}{-0.0509237382822227}
\pgfkeyssetvalue{/sea/coefs.causal/gamestyle_nameSM3DW/fml.causal}{0.126116049677774}
\pgfkeyssetvalue{/sea/coefs.causal/theme_nameCastle/fml.causal}{-0.0523856832397982}
\pgfkeyssetvalue{/sea/coefs.causal/theme_nameDesert/fml.causal}{0.0122647065868058}
\pgfkeyssetvalue{/sea/coefs.causal/theme_nameForest/fml.causal}{0.0827737015917083}
\pgfkeyssetvalue{/sea/coefs.causal/theme_nameGhost house/fml.causal}{-0.0226463920871497}
\pgfkeyssetvalue{/sea/coefs.causal/theme_nameOverworld/fml.causal}{0.142302419242461}
\pgfkeyssetvalue{/sea/coefs.causal/theme_nameSky/fml.causal}{0.0509661615946526}
\pgfkeyssetvalue{/sea/coefs.causal/theme_nameSnow/fml.causal}{0.0694591481568083}
\pgfkeyssetvalue{/sea/coefs.causal/theme_nameUnderground/fml.causal}{0.0636468325460664}
\pgfkeyssetvalue{/sea/coefs.causal/theme_nameUnderwater/fml.causal}{0.378275368011175}
\pgfkeyssetvalue{/sea/coefs.causal/game_versionV1.0.1/fml.causal}{-0.127304156773228}
\pgfkeyssetvalue{/sea/coefs.causal/game_versionV1.1.0/fml.causal}{-0.0390706154625893}
\pgfkeyssetvalue{/sea/coefs.causal/game_versionV2.0.0/fml.causal}{-0.0166927793329884}
\pgfkeyssetvalue{/sea/coefs.causal/game_versionV3.0.0/fml.causal}{0.0121595792293201}
\pgfkeyssetvalue{/sea/coefs.causal/game_versionV3.0.1/fml.causal}{0.0580085719760945}
\pgfkeyssetvalue{/sea/coefs.causal/upload_attempts/fml.causal}{-0.191122821556644}
\pgfkeyssetvalue{/sea/causal.diff/gamestyle_nameSMB3:fml.all.both}{-0.0523631285054257}
\pgfkeyssetvalue{/sea/causal.diff/gamestyle_nameSMB3:fml.user.all}{-0.0516995459774831}
\pgfkeyssetvalue{/sea/causal.diff/gamestyle_nameSMW:fml.all.both}{-0.0937139850312786}
\pgfkeyssetvalue{/sea/causal.diff/gamestyle_nameSMW:fml.user.all}{-0.0966371784671883}
\pgfkeyssetvalue{/sea/causal.diff/gamestyle_nameNSMBU:fml.all.both}{-0.0262340176960726}
\pgfkeyssetvalue{/sea/causal.diff/gamestyle_nameNSMBU:fml.user.all}{-0.0275734305239395}
\pgfkeyssetvalue{/sea/causal.diff/gamestyle_nameSM3DW:fml.all.both}{0.100467817037359}
\pgfkeyssetvalue{/sea/causal.diff/gamestyle_nameSM3DW:fml.user.all}{0.0979968024826263}
\pgfkeyssetvalue{/sea/causal.diff/theme_nameCastle:fml.all.both}{-0.0452813422700474}
\pgfkeyssetvalue{/sea/causal.diff/theme_nameCastle:fml.user.all}{-0.0431466095603515}
\pgfkeyssetvalue{/sea/causal.diff/theme_nameDesert:fml.all.both}{-0.00297400625030231}
\pgfkeyssetvalue{/sea/causal.diff/theme_nameDesert:fml.user.all}{-0.00164712245358634}
\pgfkeyssetvalue{/sea/causal.diff/theme_nameForest:fml.all.both}{0.0503368403088513}
\pgfkeyssetvalue{/sea/causal.diff/theme_nameForest:fml.user.all}{0.052891642027139}
\pgfkeyssetvalue{/sea/causal.diff/theme_nameGhost house:fml.all.both}{-0.0438229976181758}
\pgfkeyssetvalue{/sea/causal.diff/theme_nameGhost house:fml.user.all}{-0.0394645709617482}
\pgfkeyssetvalue{/sea/causal.diff/theme_nameOverworld:fml.all.both}{0.0986056265299267}
\pgfkeyssetvalue{/sea/causal.diff/theme_nameOverworld:fml.user.all}{0.103421190808892}
\pgfkeyssetvalue{/sea/causal.diff/theme_nameSky:fml.all.both}{0.0201754674897499}
\pgfkeyssetvalue{/sea/causal.diff/theme_nameSky:fml.user.all}{0.0275956478208172}
\pgfkeyssetvalue{/sea/causal.diff/theme_nameSnow:fml.all.both}{0.0362260719018768}
\pgfkeyssetvalue{/sea/causal.diff/theme_nameSnow:fml.user.all}{0.039953396442487}
\pgfkeyssetvalue{/sea/causal.diff/theme_nameUnderground:fml.all.both}{0.0319106566669227}
\pgfkeyssetvalue{/sea/causal.diff/theme_nameUnderground:fml.user.all}{0.0360119256788045}
\pgfkeyssetvalue{/sea/causal.diff/theme_nameUnderwater:fml.all.both}{0.280308302727238}
\pgfkeyssetvalue{/sea/causal.diff/theme_nameUnderwater:fml.user.all}{0.279627135194563}
\pgfkeyssetvalue{/sea/causal.diff/game_versionV1.0.1:fml.all.both}{-0.179409318677557}
\pgfkeyssetvalue{/sea/causal.diff/game_versionV1.0.1:fml.user.all}{-0.177451941691362}
\pgfkeyssetvalue{/sea/causal.diff/game_versionV1.1.0:fml.all.both}{-0.0615599035637824}
\pgfkeyssetvalue{/sea/causal.diff/game_versionV1.1.0:fml.user.all}{-0.0473000699962012}
\pgfkeyssetvalue{/sea/causal.diff/game_versionV2.0.0:fml.all.both}{-0.0216708480577948}
\pgfkeyssetvalue{/sea/causal.diff/game_versionV2.0.0:fml.user.all}{-0.012164549751524}
\pgfkeyssetvalue{/sea/causal.diff/game_versionV3.0.0:fml.all.both}{0.0271476402675078}
\pgfkeyssetvalue{/sea/causal.diff/game_versionV3.0.0:fml.user.all}{0.0306399572784977}
\pgfkeyssetvalue{/sea/causal.diff/game_versionV3.0.1:fml.all.both}{0.0692702218913085}
\pgfkeyssetvalue{/sea/causal.diff/game_versionV3.0.1:fml.user.all}{0.0734808531330322}
\pgfkeyssetvalue{/sea/causal.diff/upload_attempts:fml.all.both}{-0.172378921314361}
\pgfkeyssetvalue{/sea/causal.diff/upload_attempts:fml.user.all}{-0.173872812881465}
\pgfkeyssetvalue{/sea/causal.insignificant.vars/::N_vars}{1}
\pgfkeyssetvalue{/sea/factor/difficulty_nameEasy:Variable}{difficulty\_name}
\pgfkeyssetvalue{/sea/factor/difficulty_nameNormal:Variable}{difficulty\_name}
\pgfkeyssetvalue{/sea/factor/difficulty_nameExpert:Variable}{difficulty\_name}
\pgfkeyssetvalue{/sea/factor/difficulty_nameSuper expert:Variable}{difficulty\_name}
\pgfkeyssetvalue{/sea/factor/gamestyle_nameSMB1:Variable}{gamestyle\_name}
\pgfkeyssetvalue{/sea/factor/gamestyle_nameSMB3:Variable}{gamestyle\_name}
\pgfkeyssetvalue{/sea/factor/gamestyle_nameSMW:Variable}{gamestyle\_name}
\pgfkeyssetvalue{/sea/factor/gamestyle_nameNSMBU:Variable}{gamestyle\_name}
\pgfkeyssetvalue{/sea/factor/gamestyle_nameSM3DW:Variable}{gamestyle\_name}
\pgfkeyssetvalue{/sea/factor/theme_nameAirship:Variable}{theme\_name}
\pgfkeyssetvalue{/sea/factor/theme_nameCastle:Variable}{theme\_name}
\pgfkeyssetvalue{/sea/factor/theme_nameDesert:Variable}{theme\_name}
\pgfkeyssetvalue{/sea/factor/theme_nameForest:Variable}{theme\_name}
\pgfkeyssetvalue{/sea/factor/theme_nameGhost house:Variable}{theme\_name}
\pgfkeyssetvalue{/sea/factor/theme_nameOverworld:Variable}{theme\_name}
\pgfkeyssetvalue{/sea/factor/theme_nameSky:Variable}{theme\_name}
\pgfkeyssetvalue{/sea/factor/theme_nameSnow:Variable}{theme\_name}
\pgfkeyssetvalue{/sea/factor/theme_nameUnderground:Variable}{theme\_name}
\pgfkeyssetvalue{/sea/factor/theme_nameUnderwater:Variable}{theme\_name}
\pgfkeyssetvalue{/sea/factor/game_versionV1.0.0:Variable}{game\_version}
\pgfkeyssetvalue{/sea/factor/game_versionV1.0.1:Variable}{game\_version}
\pgfkeyssetvalue{/sea/factor/game_versionV1.1.0:Variable}{game\_version}
\pgfkeyssetvalue{/sea/factor/game_versionV2.0.0:Variable}{game\_version}
\pgfkeyssetvalue{/sea/factor/game_versionV3.0.0:Variable}{game\_version}
\pgfkeyssetvalue{/sea/factor/game_versionV3.0.1:Variable}{game\_version}
\pgfkeyssetvalue{/sea/insignificant.vars/data_99_9_makers:fml.all.both:data}{data\_99\_9\_makers}
\pgfkeyssetvalue{/sea/insignificant.vars/data_99_9_makers:fml.all.both:model}{fml.all.both}
\pgfkeyssetvalue{/sea/insignificant.vars/data_99_9_makers:fml.user.all:data}{data\_99\_9\_makers}
\pgfkeyssetvalue{/sea/insignificant.vars/data_99_9_makers:fml.user.all:model}{fml.user.all}
\pgfkeyssetvalue{/sea/insignificant.vars/data_99_9_players:fml.all.both:data}{data\_99\_9\_players}
\pgfkeyssetvalue{/sea/insignificant.vars/data_99_9_players:fml.all.both:model}{fml.all.both}
\pgfkeyssetvalue{/sea/insignificant.vars/data_99_9_players:fml.user.all:data}{data\_99\_9\_players}
\pgfkeyssetvalue{/sea/insignificant.vars/data_99_9_players:fml.user.all:model}{fml.user.all}
\pgfkeyssetvalue{/sea/causal.insignificant.vars/::model.all}{fml.all.both}

==> floats/stats_nlp.tex <==
\pgfkeyssetvalue{/sea/avg_S_i_comment:normal:neg}{0.22729908116957206}
\pgfkeyssetvalue{/sea/avg_S_i_comment:normal:neu}{0.3812437125480982}
\pgfkeyssetvalue{/sea/avg_S_i_comment:normal:pos}{0.3914572063869114}
\pgfkeyssetvalue{/sea/avg_S_i_comment:superexpert:neg}{0.2927489672055229}
\pgfkeyssetvalue{/sea/avg_S_i_comment:superexpert:neu}{0.34576174191544523}
\pgfkeyssetvalue{/sea/avg_S_i_comment:superexpert:pos}{0.3614892909555892}
\pgfkeyssetvalue{/sea/avg_S_i_comment:easy:neg}{0.2304440952549333}
\pgfkeyssetvalue{/sea/avg_S_i_comment:easy:neu}{0.40139909298002224}
\pgfkeyssetvalue{/sea/avg_S_i_comment:easy:pos}{0.3681568118484991}
\pgfkeyssetvalue{/sea/avg_S_i_comment:expert:neg}{0.24516057726171112}
\pgfkeyssetvalue{/sea/avg_S_i_comment:expert:neu}{0.3574641342448585}
\pgfkeyssetvalue{/sea/avg_S_i_comment:expert:pos}{0.39737528859551186}
\pgfkeyssetvalue{/sea/avg_S_i_level:superexpert:neg}{0.2736746457179461}
\pgfkeyssetvalue{/sea/avg_S_i_level:superexpert:neu}{0.34132598613849124}
\pgfkeyssetvalue{/sea/avg_S_i_level:superexpert:pos}{0.38499936817750385}
\pgfkeyssetvalue{/sea/avg_S_i_level:easy:neg}{0.22134664132376075}
\pgfkeyssetvalue{/sea/avg_S_i_level:easy:neu}{0.3939561202230435}
\pgfkeyssetvalue{/sea/avg_S_i_level:easy:pos}{0.3846972384984446}
\pgfkeyssetvalue{/sea/avg_S_i_level:expert:neg}{0.2294684102281084}
\pgfkeyssetvalue{/sea/avg_S_i_level:expert:neu}{0.34898462474112524}
\pgfkeyssetvalue{/sea/avg_S_i_level:expert:pos}{0.4215469651506307}
\pgfkeyssetvalue{/sea/avg_S_i_level:normal:neg}{0.20940032721228405}
\pgfkeyssetvalue{/sea/avg_S_i_level:normal:neu}{0.3657862339996966}
\pgfkeyssetvalue{/sea/avg_S_i_level:normal:pos}{0.4248134388853808}
\pgfkeyssetvalue{/sea/sent:comments:N.comments}{666}
\pgfkeyssetvalue{/sea/sent:comments:N.levels}{666}

\pgfkeyssetvalue{/sea/topics:desc:top_n_superexpert:15:Easy_p}{0.01897486145415264}
\pgfkeyssetvalue{/sea/topics:desc:top_n_superexpert:15:Normal_p}{0.022792859445652264}
\pgfkeyssetvalue{/sea/topics:desc:top_n_superexpert:15:Expert_p}{0.03743632867642162}
\pgfkeyssetvalue{/sea/topics:desc:top_n_superexpert:15:Super_Expert_p}{0.044510495282172526}
\pgfkeyssetvalue{/sea/topics:desc:top_n_superexpert:13:Easy_p}{0.00927723006718165}
\pgfkeyssetvalue{/sea/topics:desc:top_n_superexpert:13:Normal_p}{0.015936257450132676}
\pgfkeyssetvalue{/sea/topics:desc:top_n_superexpert:13:Expert_p}{0.025467446470603845}
\pgfkeyssetvalue{/sea/topics:desc:top_n_superexpert:13:Super_Expert_p}{0.03150891532517278}
\pgfkeyssetvalue{/sea/topics:desc:top_n_superexpert:32:Easy_p}{0.0021759813794909543}
\pgfkeyssetvalue{/sea/topics:desc:top_n_superexpert:32:Normal_p}{0.004934653759992064}
\pgfkeyssetvalue{/sea/topics:desc:top_n_superexpert:32:Expert_p}{0.01562712361834514}
\pgfkeyssetvalue{/sea/topics:desc:top_n_superexpert:32:Super_Expert_p}{0.028026038019445466}
\pgfkeyssetvalue{/sea/topics:desc:top_n_superexpert:56:Easy_p}{0.0007040813933942502}
\pgfkeyssetvalue{/sea/topics:desc:top_n_superexpert:56:Normal_p}{0.001476593563746683}
\pgfkeyssetvalue{/sea/topics:desc:top_n_superexpert:56:Expert_p}{0.0060618727965133}
\pgfkeyssetvalue{/sea/topics:desc:top_n_superexpert:56:Super_Expert_p}{0.023710633079849854}
\pgfkeyssetvalue{/sea/topics:desc:top_n_superexpert:25:Easy_p}{0.0036181593555475633}
\pgfkeyssetvalue{/sea/topics:desc:top_n_superexpert:25:Normal_p}{0.005904720966181978}
\pgfkeyssetvalue{/sea/topics:desc:top_n_superexpert:25:Expert_p}{0.010717521059525479}
\pgfkeyssetvalue{/sea/topics:desc:top_n_superexpert:25:Super_Expert_p}{0.014540525743251348}

\pgfkeyssetvalue{/sea/topics:desc:top_n_easy:0:Easy_p}{0.09514609854035208}
\pgfkeyssetvalue{/sea/topics:desc:top_n_easy:0:Normal_p}{0.07571318745815113}
\pgfkeyssetvalue{/sea/topics:desc:top_n_easy:0:Expert_p}{0.05896558838069753}
\pgfkeyssetvalue{/sea/topics:desc:top_n_easy:0:Super_Expert_p}{0.04750021274566998}
\pgfkeyssetvalue{/sea/topics:desc:top_n_easy:5:Easy_p}{0.03856496851613525}
\pgfkeyssetvalue{/sea/topics:desc:top_n_easy:5:Normal_p}{0.03463640045961429}
\pgfkeyssetvalue{/sea/topics:desc:top_n_easy:5:Expert_p}{0.03572416773112684}
\pgfkeyssetvalue{/sea/topics:desc:top_n_easy:5:Super_Expert_p}{0.03689471293688477}
\pgfkeyssetvalue{/sea/topics:desc:top_n_easy:30:Easy_p}{0.023573186651911337}
\pgfkeyssetvalue{/sea/topics:desc:top_n_easy:30:Normal_p}{0.01807023997487001}
\pgfkeyssetvalue{/sea/topics:desc:top_n_easy:30:Expert_p}{0.009781301491399396}
\pgfkeyssetvalue{/sea/topics:desc:top_n_easy:30:Super_Expert_p}{0.006546414953508662}
\pgfkeyssetvalue{/sea/topics:desc:top_n_easy:16:Easy_p}{0.01887347637546032}
\pgfkeyssetvalue{/sea/topics:desc:top_n_easy:16:Normal_p}{0.01782265997635797}
\pgfkeyssetvalue{/sea/topics:desc:top_n_easy:16:Expert_p}{0.017664172788553537}
\pgfkeyssetvalue{/sea/topics:desc:top_n_easy:16:Super_Expert_p}{0.016101002416585755}
\pgfkeyssetvalue{/sea/topics:desc:top_n_easy:40:Easy_p}{0.01851417029853117}
\pgfkeyssetvalue{/sea/topics:desc:top_n_easy:40:Normal_p}{0.010128253879028859}
\pgfkeyssetvalue{/sea/topics:desc:top_n_easy:40:Expert_p}{0.007291033247436497}
\pgfkeyssetvalue{/sea/topics:desc:top_n_easy:40:Super_Expert_p}{0.005687230030871191}

\pgfkeyssetvalue{/sea/sent:titledesc:N.levels}{10689031}
\pgfkeyssetvalue{/sea/sent:comments:N.comments}{1996367}
\pgfkeyssetvalue{/sea/sent:comments:N.levels}{100148}

\pgfkeyssetvalue{/sea/topics:comm:top_n_superexpert:0:Easy_p}{0.39296127679165177}
\pgfkeyssetvalue{/sea/topics:comm:top_n_superexpert:0:Normal_p}{0.4545666491810923}
\pgfkeyssetvalue{/sea/topics:comm:top_n_superexpert:0:Expert_p}{0.4887853370611992}
\pgfkeyssetvalue{/sea/topics:comm:top_n_superexpert:0:Super_Expert_p}{0.5566206183629357}
\pgfkeyssetvalue{/sea/topics:comm:top_n_superexpert:5:Easy_p}{0.09821474244206865}
\pgfkeyssetvalue{/sea/topics:comm:top_n_superexpert:5:Normal_p}{0.12155388471177946}
\pgfkeyssetvalue{/sea/topics:comm:top_n_superexpert:5:Expert_p}{0.17639018328673503}
\pgfkeyssetvalue{/sea/topics:comm:top_n_superexpert:5:Super_Expert_p}{0.2224414998590358}
\pgfkeyssetvalue{/sea/topics:comm:top_n_superexpert:10:Easy_p}{0.07005473425750679}
\pgfkeyssetvalue{/sea/topics:comm:top_n_superexpert:10:Normal_p}{0.07920965203706942}
\pgfkeyssetvalue{/sea/topics:comm:top_n_superexpert:10:Expert_p}{0.11102826964895932}
\pgfkeyssetvalue{/sea/topics:comm:top_n_superexpert:10:Super_Expert_p}{0.1380509350624941}
\pgfkeyssetvalue{/sea/topics:comm:top_n_superexpert:50:Easy_p}{0.014860095145531741}
\pgfkeyssetvalue{/sea/topics:comm:top_n_superexpert:50:Normal_p}{0.026228361601678615}
\pgfkeyssetvalue{/sea/topics:comm:top_n_superexpert:50:Expert_p}{0.04137931034482759}
\pgfkeyssetvalue{/sea/topics:comm:top_n_superexpert:50:Super_Expert_p}{0.08852551451931209}
\pgfkeyssetvalue{/sea/topics:comm:top_n_superexpert:38:Easy_p}{0.037776868382014425}
\pgfkeyssetvalue{/sea/topics:comm:top_n_superexpert:38:Normal_p}{0.03820598006644518}
\pgfkeyssetvalue{/sea/topics:comm:top_n_superexpert:38:Expert_p}{0.04628766697732215}
\pgfkeyssetvalue{/sea/topics:comm:top_n_superexpert:38:Super_Expert_p}{0.08814960999906024}

\pgfkeyssetvalue{/sea/topics:comm:top_n_easy:-1:Easy_p}{0.9974679011714155}
\pgfkeyssetvalue{/sea/topics:comm:top_n_easy:-1:Normal_p}{0.9970565949758117}
\pgfkeyssetvalue{/sea/topics:comm:top_n_easy:-1:Expert_p}{0.9962100031065549}
\pgfkeyssetvalue{/sea/topics:comm:top_n_easy:-1:Super_Expert_p}{0.997368668358237}
\pgfkeyssetvalue{/sea/topics:comm:top_n_easy:1:Easy_p}{0.2411120773441097}
\pgfkeyssetvalue{/sea/topics:comm:top_n_easy:1:Normal_p}{0.21489770938975347}
\pgfkeyssetvalue{/sea/topics:comm:top_n_easy:1:Expert_p}{0.1636533084808947}
\pgfkeyssetvalue{/sea/topics:comm:top_n_easy:1:Super_Expert_p}{0.1242364439432384}
\pgfkeyssetvalue{/sea/topics:comm:top_n_easy:2:Easy_p}{0.169471584224257}
\pgfkeyssetvalue{/sea/topics:comm:top_n_easy:2:Normal_p}{0.14373142157719881}
\pgfkeyssetvalue{/sea/topics:comm:top_n_easy:2:Expert_p}{0.14290152221186705}
\pgfkeyssetvalue{/sea/topics:comm:top_n_easy:2:Super_Expert_p}{0.1490461422798609}
\pgfkeyssetvalue{/sea/topics:comm:top_n_easy:3:Easy_p}{0.16146605964499464}
\pgfkeyssetvalue{/sea/topics:comm:top_n_easy:3:Normal_p}{0.14999708573759982}
\pgfkeyssetvalue{/sea/topics:comm:top_n_easy:3:Expert_p}{0.13793103448275865}
\pgfkeyssetvalue{/sea/topics:comm:top_n_easy:3:Super_Expert_p}{0.11737618644864203}
\pgfkeyssetvalue{/sea/topics:comm:top_n_easy:4:Easy_p}{0.16115913857486316}
\pgfkeyssetvalue{/sea/topics:comm:top_n_easy:4:Normal_p}{0.14309028384915778}
\pgfkeyssetvalue{/sea/topics:comm:top_n_easy:4:Expert_p}{0.12581547064305687}
\pgfkeyssetvalue{/sea/topics:comm:top_n_easy:4:Super_Expert_p}{0.09444601071327882}
\pgfkeyssetvalue{/sea/topics:comm:top_n_easy:8:Easy_p}{0.12420072637986598}
\pgfkeyssetvalue{/sea/topics:comm:top_n_easy:8:Normal_p}{0.09177012298187329}
\pgfkeyssetvalue{/sea/topics:comm:top_n_easy:8:Expert_p}{0.09388008698353527}
\pgfkeyssetvalue{/sea/topics:comm:top_n_easy:8:Super_Expert_p}{0.09801710365567146}

\pgfkeyssetvalue{/sea/avg_SR_i:superexpert:neg}{0.26481370814623006}
\pgfkeyssetvalue{/sea/avg_SR_i:superexpert:neu}{0.36101630209098995}
\pgfkeyssetvalue{/sea/avg_SR_i:superexpert:pos}{0.3741699897627799}
\pgfkeyssetvalue{/sea/avg_SR_i:easy:neg}{0.1977866141420175}
\pgfkeyssetvalue{/sea/avg_SR_i:easy:neu}{0.44031133739031253}
\pgfkeyssetvalue{/sea/avg_SR_i:easy:pos}{0.3619020484676698}
\pgfkeyssetvalue{/sea/avg_SR_i:expert:neg}{0.2124844869567172}
\pgfkeyssetvalue{/sea/avg_SR_i:expert:neu}{0.37798632169603835}
\pgfkeyssetvalue{/sea/avg_SR_i:expert:pos}{0.4095291913472441}
\pgfkeyssetvalue{/sea/avg_SR_i:normal:neg}{0.18645783660401782}
\pgfkeyssetvalue{/sea/avg_SR_i:normal:neu}{0.4048855193474178}
\pgfkeyssetvalue{/sea/avg_SR_i:normal:pos}{0.40865664404856433}

\pgfkeyssetvalue{/sea/topics:comm:0:sent_pos:avg}{0.665554}
\pgfkeyssetvalue{/sea/topics:comm:38:sent_neg:avg}{0.459021}
\pgfkeyssetvalue{/sea/topics:comm:3:sent_pos:avg}{0.624591}
\pgfkeyssetvalue{/sea/topics:comm:4:sent_pos:avg}{0.857831}
\pgfkeyssetvalue{/sea/topics:comm:8:sent_neg:avg}{0.341711}

\pgfkeyssetvalue{/sea/topics:comm:2:sent_neg:avg}{0.202001}

\pgfkeyssetvalue{/sea/d_S_i_comment:easy:neg}{-0.02512335809691173}
\pgfkeyssetvalue{/sea/d_S_i_comment:normal:neg}{-0.0942340022722234}
\pgfkeyssetvalue{/sea/d_S_i_comment:expert:neg}{0.030697667728079983}
\pgfkeyssetvalue{/sea/d_S_i_comment:superexpert:neg}{0.24286592404094834}
\pgfkeyssetvalue{/sea/d_S_i_comment:easy:pos}{-0.08635772710661452}
\pgfkeyssetvalue{/sea/d_S_i_comment:normal:pos}{0.07954936541916316}
\pgfkeyssetvalue{/sea/d_S_i_comment:expert:pos}{0.05780053929567147}
\pgfkeyssetvalue{/sea/d_S_i_comment:superexpert:pos}{-0.054353446193786514}

\pgfkeyssetvalue{/sea/d_SR_i_comment:easy:neg}{-0.04134384967419905}
\pgfkeyssetvalue{/sea/d_SR_i_comment:normal:neg}{-0.086964355370354}
\pgfkeyssetvalue{/sea/d_SR_i_comment:expert:neg}{0.043784077907293266}
\pgfkeyssetvalue{/sea/d_SR_i_comment:superexpert:neg}{0.24768632509619698}
\pgfkeyssetvalue{/sea/d_SR_i_comment:easy:pos}{-0.09412821072599066}
\pgfkeyssetvalue{/sea/d_SR_i_comment:normal:pos}{0.07164135233539722}
\pgfkeyssetvalue{/sea/d_SR_i_comment:expert:pos}{0.06456537927461241}
\pgfkeyssetvalue{/sea/d_SR_i_comment:superexpert:pos}{-0.025731977244347913}

\pgfkeyssetvalue{/sea/cliffsdelta:S_i:comment}{0.09335058085813255}
\pgfkeyssetvalue{/sea/cliffsdelta:S_i:level}{0.19272765469357053}
\pgfkeyssetvalue{/sea/cliffsdelta:SR_i}{0.24768632509619698}

==> floats/tab_comm_topics.tex <==
\setlength{\tabcolsep}{4pt}
\begin{tabular}{llrrrrc}
  \toprule
  \multicolumn{2}{c}{topic} &
  \multicolumn{4}{c}{frequency per \textcolor[HTML]{E7298A}{difficulty}} \\
  \cmidrule(l{3pt}r{3pt}){1-2} \cmidrule(l{3pt}r{3pt}){3-6} 
  \# & \multicolumn{1}{c}{top-4 topic words} & \multicolumn{1}{c}{\rotatebox{-90}{easy}} & \multicolumn{1}{c}{\rotatebox{-90}{normal}} & \multicolumn{1}{c}{\rotatebox{-90}{expert}} & \multicolumn{1}{c}{\rotatebox{-90}{super expert}} \\
  \toprule
  \#0 & [level, great level, good level]  & \n[2]{topics:comm:top_n_superexpert:0:Easy_p}[100]| & \n[2]{topics:comm:top_n_superexpert:0:Normal_p}[100]| & \n[2]{topics:comm:top_n_superexpert:0:Expert_p}[100]| & \n[2]{topics:comm:top_n_superexpert:0:Super_Expert_p}[100]| \\ 
  \#5 & [hard, easy, beat, challenge]  & \n[2]{topics:comm:top_n_superexpert:5:Easy_p}[100]| & \n[2]{topics:comm:top_n_superexpert:5:Normal_p}[100]| & \n[2]{topics:comm:top_n_superexpert:5:Expert_p}[100]| & \n[2]{topics:comm:top_n_superexpert:5:Super_Expert_p}[100]| \\ 
  \#10 & [jump, spin, jumping, jumped]  & \n[2]{topics:comm:top_n_superexpert:10:Easy_p}[100]| & \n[2]{topics:comm:top_n_superexpert:10:Normal_p}[100]| & \n[2]{topics:comm:top_n_superexpert:10:Expert_p}[100]| & \n[2]{topics:comm:top_n_superexpert:10:Super_Expert_p}[100]| \\ 
  \#50 & [shell, jump, throw, double]  & \n[2]{topics:comm:top_n_superexpert:50:Easy_p}[100]| & \n[2]{topics:comm:top_n_superexpert:50:Normal_p}[100]| & \n[2]{topics:comm:top_n_superexpert:50:Expert_p}[100]| & \n[2]{topics:comm:top_n_superexpert:50:Super_Expert_p}[100]| \\ 
  \#38 & [troll, bully, mad, lad]  & \n[2]{topics:comm:top_n_superexpert:38:Easy_p}[100]| & \n[2]{topics:comm:top_n_superexpert:38:Normal_p}[100]| & \n[2]{topics:comm:top_n_superexpert:38:Expert_p}[100]| & \n[2]{topics:comm:top_n_superexpert:38:Super_Expert_p}[100]| \\
  \bottomrule
  \#1 & [mario, toad, bros, maker]  & \n[2]{topics:comm:top_n_easy:1:Easy_p}[100]| & \n[2]{topics:comm:top_n_easy:1:Normal_p}[100]| & \n[2]{topics:comm:top_n_easy:1:Expert_p}[100]| & \n[2]{topics:comm:top_n_easy:1:Super_Expert_p}[100]| \\ 
  \#2 & [nintendo, switch, minecraft]  & \n[2]{topics:comm:top_n_easy:2:Easy_p}[100]| & \n[2]{topics:comm:top_n_easy:2:Normal_p}[100]| & \n[2]{topics:comm:top_n_easy:2:Expert_p}[100]| & \n[2]{topics:comm:top_n_easy:2:Super_Expert_p}[100]| \\ 
  \#3 & [course, great course, fun course]  & \n[2]{topics:comm:top_n_easy:3:Easy_p}[100]| & \n[2]{topics:comm:top_n_easy:3:Normal_p}[100]| & \n[2]{topics:comm:top_n_easy:3:Expert_p}[100]| & \n[2]{topics:comm:top_n_easy:3:Super_Expert_p}[100]| \\ 
  \#4 & [awesome, good job, thanks]  & \n[2]{topics:comm:top_n_easy:4:Easy_p}[100]| & \n[2]{topics:comm:top_n_easy:4:Normal_p}[100]| & \n[2]{topics:comm:top_n_easy:4:Expert_p}[100]| & \n[2]{topics:comm:top_n_easy:4:Super_Expert_p}[100]| \\ 
  \#8 & [brain, eyes, pain, dad]  & \n[2]{topics:comm:top_n_easy:8:Easy_p}[100]| & \n[2]{topics:comm:top_n_easy:8:Normal_p}[100]| & \n[2]{topics:comm:top_n_easy:8:Expert_p}[100]| & \n[2]{topics:comm:top_n_easy:8:Super_Expert_p}[100]| \\ 
  \bottomrule
\end{tabular}
\setlength{\tabcolsep}{6pt}


==> floats/tab_comments_sent_overall.tex <==
\setlength{\tabcolsep}{4pt}
\begin{tabular}{c *{4}{rr}}
  \toprule
  \multicolumn{1}{c}{\textcolor[HTML]{E7298A}{difficulty}} & \multicolumn{2}{c}{$d[S_i^x]$} & \multicolumn{2}{c}{$d[\SR_i^x]$} & \multicolumn{2}{c}{$\overline{S_i(\{x\})}$}  & \multicolumn{2}{c}{$\overline{\SR_i(\{x\})}$}\\

 $x$ & $-$ & $+$ & $-$ & $+$  & $-$ & $+$ & $-$ & $+$\\
  \cmidrule(l{3pt}r{3pt}){1-1} \cmidrule(l{3pt}r{3pt}){2-3}  \cmidrule(l{3pt}r{3pt}){4-5} \cmidrule(l{3pt}r{3pt}){6-7} \cmidrule(l{3pt}r{3pt}){8-9} 
  easy & \n[2]{d_S_i_comment:easy:neg} & \n[2]{d_S_i_comment:easy:pos} & \n[2]{d_SR_i_comment:easy:neg} & \n[2]{d_SR_i_comment:easy:pos} & \n[2]{avg_S_i_level:easy:neg} & \n[2]{avg_S_i_level:easy:pos} & \n[2]{avg_SR_i:easy:neg} & \n[2]{avg_SR_i:easy:pos}\\
  normal & \n[2]{d_S_i_comment:normal:neg} & \n[2]{d_S_i_comment:normal:pos} & \n[2]{d_SR_i_comment:normal:neg} & \n[2]{d_SR_i_comment:normal:pos} & \n[2]{avg_S_i_level:normal:neg} & \n[2]{avg_S_i_level:normal:pos} & \n[2]{avg_SR_i:normal:neg} & \n[2]{avg_SR_i:normal:pos} \\
  expert & \n[2]{d_S_i_comment:expert:neg} & \n[2]{d_S_i_comment:expert:pos} & \n[2]{d_SR_i_comment:expert:neg} & \n[2]{d_SR_i_comment:expert:pos} & \n[2]{avg_S_i_level:expert:neg} & \n[2]{avg_S_i_level:expert:pos} & \n[2]{avg_SR_i:expert:neg} & \n[2]{avg_SR_i:expert:pos}\\
  super expert & \n[2]{d_S_i_comment:superexpert:neg} & \n[2]{d_S_i_comment:superexpert:pos} & \n[2]{d_SR_i_comment:superexpert:neg} & \n[2]{d_SR_i_comment:superexpert:pos} & \n[2]{avg_S_i_level:superexpert:neg} & \n[2]{avg_S_i_level:superexpert:pos}& \n[2]{avg_SR_i:superexpert:neg} & \n[2]{avg_SR_i:superexpert:pos} \\
  \bottomrule
  \end{tabular}
\setlength{\tabcolsep}{6pt}


==> floats/tab_desc_topics.tex <==
\setlength{\tabcolsep}{4.5pt}
\begin{tabular}{llccccccccccccccccccccccc}
  \toprule
  \multicolumn{2}{c}{topic} &
  \multicolumn{4}{c}{frequency per \textcolor[HTML]{E7298A}{difficulty}} \\
  \cmidrule(l{3pt}r{3pt}){1-2} \cmidrule(l{3pt}r{3pt}){3-6} 
  \# & \multicolumn{1}{c}{top-4 topic words} & \rotatebox{-90}{easy} & \rotatebox{-90}{normal} & \rotatebox{-90}{expert} & \rotatebox{-90}{super expert} \\
  \toprule
  \#15 & [speed, speedrun, run, seconds]  & \n[2]{topics:desc:top_n_superexpert:15:Easy_p}[100]| & \n[2]{topics:desc:top_n_superexpert:15:Normal_p}[100]| & \n[2]{topics:desc:top_n_superexpert:15:Expert_p}[100]| & \n[2]{topics:desc:top_n_superexpert:15:Super_Expert_p}[100]| \\ 
  \#13 & [jump, jumps, jumping, long]  & \n[2]{topics:desc:top_n_superexpert:13:Easy_p}[100]| & \n[2]{topics:desc:top_n_superexpert:13:Normal_p}[100]| & \n[2]{topics:desc:top_n_superexpert:13:Expert_p}[100]| & \n[2]{topics:desc:top_n_superexpert:13:Super_Expert_p}[100]| \\ 
  \#32 & [level, lol, sorry, little]  & \n[2]{topics:desc:top_n_superexpert:32:Easy_p}[100]| & \n[2]{topics:desc:top_n_superexpert:32:Normal_p}[100]| & \n[2]{topics:desc:top_n_superexpert:32:Expert_p}[100]| & \n[2]{topics:desc:top_n_superexpert:32:Super_Expert_p}[100]| \\ 
  \#56 & [practice, tricks, jumps, basic]  & \n[2]{topics:desc:top_n_superexpert:56:Easy_p}[100]| & \n[2]{topics:desc:top_n_superexpert:56:Normal_p}[100]| & \n[2]{topics:desc:top_n_superexpert:56:Expert_p}[100]| & \n[2]{topics:desc:top_n_superexpert:56:Super_Expert_p}[100]| \\ 
  \#25 & [ride, spin, run, victory]  & \n[2]{topics:desc:top_n_superexpert:25:Easy_p}[100]| & \n[2]{topics:desc:top_n_superexpert:25:Normal_p}[100]| & \n[2]{topics:desc:top_n_superexpert:25:Expert_p}[100]| & \n[2]{topics:desc:top_n_superexpert:25:Super_Expert_p}[100]| \\
  \bottomrule
  \#0 & [maker, super, bros, 11]  & \n[2]{topics:desc:top_n_easy:0:Easy_p}[100]| & \n[2]{topics:desc:top_n_easy:0:Normal_p}[100]| & \n[2]{topics:desc:top_n_easy:0:Expert_p}[100]| & \n[2]{topics:desc:top_n_easy:0:Super_Expert_p}[100]| \\ 
  \#5 & [level, level easy, easy level]  & \n[2]{topics:desc:top_n_easy:5:Easy_p}[100]| & \n[2]{topics:desc:top_n_easy:5:Normal_p}[100]| & \n[2]{topics:desc:top_n_easy:5:Expert_p}[100]| & \n[2]{topics:desc:top_n_easy:5:Super_Expert_p}[100]| \\ 
  \#30 & [world, 11, 12, 13]  & \n[2]{topics:desc:top_n_easy:30:Easy_p}[100]| & \n[2]{topics:desc:top_n_easy:30:Normal_p}[100]| & \n[2]{topics:desc:top_n_easy:30:Expert_p}[100]| & \n[2]{topics:desc:top_n_easy:30:Super_Expert_p}[100]| \\ 
  \#16 & [hard, easy, try, impossible]  & \n[2]{topics:desc:top_n_easy:16:Easy_p}[100]| & \n[2]{topics:desc:top_n_easy:16:Normal_p}[100]| & \n[2]{topics:desc:top_n_easy:16:Expert_p}[100]| & \n[2]{topics:desc:top_n_easy:16:Super_Expert_p}[100]| \\ 
  \#40 & [water, dangerous, madness, life]  & \n[2]{topics:desc:top_n_easy:40:Easy_p}[100]| & \n[2]{topics:desc:top_n_easy:40:Normal_p}[100]| & \n[2]{topics:desc:top_n_easy:40:Expert_p}[100]| & \n[2]{topics:desc:top_n_easy:40:Super_Expert_p}[100]| \\
  \bottomrule
\end{tabular}
\setlength{\tabcolsep}{6pt}


==> floats/tab_factor.tex <==
\begin{tabular}{ccccccccccccccccccccccccc}
\toprule
\multicolumn{4}{c}{\textcolor[HTML]{E7298A}{difficulty}} & \multicolumn{5}{c}{\textcolor[HTML]{7570B3}{style}} & \multicolumn{10}{c}{\textcolor[HTML]{7570B3}{theme}} & \multicolumn{6}{c}{\textcolor[HTML]{7570B3}{version}} \\
\cmidrule(l{3pt}r{3pt}){1-4} \cmidrule(l{3pt}r{3pt}){5-9} \cmidrule(l{3pt}r{3pt}){10-19} \cmidrule(l{3pt}r{3pt}){20-25}
\rotatebox{-90}{easy} & \rotatebox{-90}{normal} & \rotatebox{-90}{expert} & \rotatebox{-90}{super expert} & \rotatebox{-90}{SMB1} & \rotatebox{-90}{SMB3} & \rotatebox{-90}{SMW} & \rotatebox{-90}{NSMBU} & \rotatebox{-90}{SM3DW} & \rotatebox{-90}{airship} & \rotatebox{-90}{castle} & \rotatebox{-90}{desert} & \rotatebox{-90}{forest} & \rotatebox{-90}{ghost} & \rotatebox{-90}{overworld} & \rotatebox{-90}{sky} & \rotatebox{-90}{snow} & \rotatebox{-90}{underground} & \rotatebox{-90}{water} & \rotatebox{-90}{1.0.0} & \rotatebox{-90}{1.0.1} & \rotatebox{-90}{1.1.0} & \rotatebox{-90}{2.0.0} & \rotatebox{-90}{3.0.0} & \rotatebox{-90}{3.0.1}\\
33 & 44 & 16 & 8 & 14 & 8 & 17 & 33 & 28 & 6 & 15 & 7 & 8 & 5 & 31 & 10 & 9 & 7 & 2 & 0 & 24 & 5 & 15 & 14 & 42\\
\bottomrule
\end{tabular}


==> floats/tab_numeric.tex <==
\begin{tabular}{lrrrrrrrrrrrrrrr}
\toprule
\multicolumn{1}{c}{ } & \multicolumn{7}{c}{\textcolor[HTML]{1B9E77}{plays}} & \multicolumn{3}{c}{\textcolor[HTML]{D95F02}{timing}} & \multicolumn{5}{c}{\textcolor[HTML]{66A61E}{user}} \\
\cmidrule(l{3pt}r{3pt}){2-8} \cmidrule(l{3pt}r{3pt}){9-11} \cmidrule(l{3pt}r{3pt}){12-16}
\rotatebox{-90}{ } & \rotatebox{-90}{\textcolor[HTML]{1B9E77}{attempts}} & \rotatebox{-90}{\textcolor[HTML]{1B9E77}{boos}} & \rotatebox{-90}{\textcolor[HTML]{1B9E77}{clear rate}} & \rotatebox{-90}{\textcolor[HTML]{1B9E77}{clears}} & \rotatebox{-90}{\textcolor[HTML]{1B9E77}{comments}} & \rotatebox{-90}{\textcolor[HTML]{1B9E77}{likes}} & \rotatebox{-90}{\textcolor[HTML]{1B9E77}{players}} & \rotatebox{-90}{\textcolor[HTML]{D95F02}{autoscroll: speed}} & \rotatebox{-90}{\textcolor[HTML]{D95F02}{timer}} & \rotatebox{-90}{\textcolor[HTML]{D95F02}{world record}} & \rotatebox{-90}{\textcolor[HTML]{66A61E}{cleared}} & \rotatebox{-90}{\textcolor[HTML]{66A61E}{first clears}} & \rotatebox{-90}{\textcolor[HTML]{66A61E}{maker points}} & \rotatebox{-90}{\textcolor[HTML]{66A61E}{records}} & \rotatebox{-90}{\textcolor[HTML]{66A61E}{uploaded}}\\
\midrule
min & \numprint{0} & \numprint{0} & \numprint{0.00} & \numprint{0} & \numprint{0} & \numprint{0} & \numprint{0} & \numprint{0} & \numprint{10} & \numprint{-0} & \numprint{0} & \numprint{0} & \numprint{0} & \numprint{0} & \numprint{0}\\
25\% & \numprint{22} & \numprint{0} & \numprint{0.10} & \numprint{4} & \numprint{0} & \numprint{0} & \numprint{10} & \numprint{0} & \numprint{300} & \numprint{10} & \numprint{80} & \numprint{1} & \numprint{780} & \numprint{0} & \numprint{10}\\
50\% & \numprint{54} & \numprint{1} & \numprint{0.25} & \numprint{10} & \numprint{0} & \numprint{1} & \numprint{21} & \numprint{0} & \numprint{300} & \numprint{21} & \numprint{219} & \numprint{4} & \numprint{1599} & \numprint{2} & \numprint{25}\\
75\% & \numprint{127} & \numprint{2} & \numprint{0.50} & \numprint{28} & \numprint{1} & \numprint{4} & \numprint{48} & \numprint{0} & \numprint{300} & \numprint{44} & \numprint{534} & \numprint{11} & \numprint{2441} & \numprint{7} & \numprint{52}\\
99\% & \numprint{1431} & \numprint{15} & \numprint{1.00} & \numprint{247} & \numprint{13} & \numprint{49} & \numprint{325} & \numprint{0} & \numprint{500} & \numprint{258} & \numprint{4502} & \numprint{215} & \numprint{7687} & \numprint{268} & \numprint{100}\\
99.99\% & \numprint{142163} & \numprint{576} & \numprint{1.00} & \numprint{15557} & \numprint{906} & \numprint{4590} & \numprint{18171} & \numprint{2} & \numprint{500} & \numprint{2628} & \numprint{57813} & \numprint{7803} & \numprint{22633} & \numprint{10674} & \numprint{100}\\
max & \numprint{67895905} & \numprint{37886} & \numprint{1.00} & \numprint{1804430} & \numprint{120515} & \numprint{564890} & \numprint{1302862} & \numprint{2} & \numprint{500} & \numprint{6000} & \numprint{513124} & \numprint{67102} & \numprint{29100} & \numprint{105379} & \numprint{100}\\
\bottomrule
\end{tabular}


==> floats/var-palette.tex <==
\definecolor{plays}{HTML}{1B9E77}
\definecolor{timing}{HTML}{D95F02}
\definecolor{style}{HTML}{7570B3}
\definecolor{difficulty}{HTML}{E7298A}
\definecolor{user}{HTML}{66A61E}
\definecolor{negative}{HTML}{7b3294}
\definecolor{positive}{HTML}{008837}


==> smm2-easyhard-rw.tex <==


\section{Related Work}
\label{sec:rw}

Difficulty is a fundamental characteristic
of videogame experience~\cite{ChenFlowGames2007},
which has been investigated in disparate ways~\cite{alexander2013investigation,aponte2009scaling,aponte2011difficulty}.
For \emph{platformers} specifically,
a very recent work
introduced a model to automatically evaluate their difficulty
based on a level's structure~\cite{Francillette2025};
applying this model to \smm levels is an interesting future work direction.
The \emph{Platformer Experience Dataset (PED)}~\cite{karpouzis2015a}
corpus collects various kinds of data
that capture the experience of Super Mario Bros.\ players
with rankings, game content recordings, and visual 
recordings of players.
Another approach~\cite{Rosa2021a} measures difficulty in platformers
through 
a machine learning model trained on both performance telemetry data
and emotional data estimated from electrodermal activity.
All these approaches focus on precisely measuring
the difficulty of individual levels and player runs.
In contrast, 
our paper mainly analyzes \emph{metadata},
such as a level's style or description;
by focusing on such data,
we have access to large amounts of user information,
including measures, such as the clear rate,
that are normally not available for single-player games.
Our approach is also justified by the specific game
we targeted:
in \smm, (some) players are also level designers,
which adds an interesting dimension to the analysis.
While metadata is arguably more coarse-grained than, say, a level's detailed structure,
our work demonstrated that it can provide complementary, broad-stroke insights.

A very different angle to analyze games
is as models of computation~\cite{ALOUPIS2015135,abel_et_al:LIPIcs.FUN.2024.1,jcai20:angrybirds}.
For example,
the undecidability~\cite{mithardnessgroup_et_al:LIPIcs.FUN.2024.22}
and the computational complexity~\cite{ALOUPIS2015135,demaine_et_al:LIPIcs.FUN.2016.13}
of classic Nintendo games,
in particular Mario games,
has been painstakingly studied.
NLP sentiment analysis has been applied to artifacts related to videogames,
including reviews~\cite{ViggiatoIEEE22}, chats~\cite{THOMPSON2017149}, and
player speech~\cite{sykownik2019can}. Other work 
focused on specific (sub)genres, like Virtual Reality~\cite{Guzsvinecz24}
or ``Souls-like'' games~\cite{Sicheng2024a};
their findings include that player negative emotions 
can also be influenced by cultural elements. 







==> smm2-easyhard-sec-nlp.tex <==


\section{NLP Analysis}
\label{sec:nlp}


We leverage NLP (natural language processing) techniques to analyze how level titles and descriptions 
(\autoref{sec:nlp:titledesc}), and comments (\autoref{sec:nlp:comments}) relate to a level's \vg*{difficulty}[difficulty].

\subsection{Titles and Descriptions}
\label{sec:nlp:titledesc}
 
The title and the description of a level represent the creator's
highlights of the level's content. To study how 
this correlates with the level's \vg*{difficulty}[difficulty],
we leverage \bertopic, a 
topic modeling approach~\cite{grootendorst2022bertopic}. \bertopic
extracts latent topics from a collection of documents; in our case, each level is a document
consisting of the concatenation of the level's title and description. The base
\bertopic algorithm uses pre-trained transformer-based language models to build
 document embeddings, which are clustered by similarity to derive latent topics. Then, \bertopic
 derives topic representations according to their class-based term frequency-inverse document frequency (TF-IDF). We configured \bertopic to use words and bigrams as topics;
 in practice, a topic is a collection of words that
 tend to occur together in several documents.
 In the following, ``topic-word'' refers to any of the words that
 characterize a topic.


Consistently with the game's worldwide popularity,
\smm titles and descriptions are written in many different languages.
We focus on English text, which is the most widely used language.
Since the \smm dataset has no information about language,
we use the \textsc{Lingua} language detector~\footnote{See \url{https://github.com/pemistahl/lingua-py}.}, obtaining a total of \n{sent:titledesc:N.levels} levels with title and descriptions in English.

To understand which topics characterize each difficulty, we 
calculate the relative frequency of a topic $t$ for each \vg*{difficulty}[difficulty] $d$ (easy, normal, expert, super expert)
as the 
fraction of levels with difficulty $d$
whose title/description matches topic $t$.
Based on this metric,
we call topic $t$
a \emph{characterizing topics} for \vg*{difficulty}[difficulty] $d$
if $t$'s frequency in levels of difficulty $d$
is higher than its frequency in levels of other difficulties.
Of the total 179 topics extracted 
with \bertopic, 52 are characterizing for \emph{super expert}, 20 for \emph{expert}, 37 for \emph{normal}, and 70 for \emph{easy}.
\autoref{tab:desc:topics} shows the top-5 characterizing topics for the \emph{super expert} and \emph{easy} difficulties. 

\begin{table}[h]
  \centering
  \scriptsize
    \setlength{\tabcolsep}{4.5pt}
\begin{tabular}{llccccccccccccccccccccccc}
  \toprule
  \multicolumn{2}{c}{topic} &
  \multicolumn{4}{c}{frequency per \textcolor[HTML]{E7298A}{difficulty}} \\
  \cmidrule(l{3pt}r{3pt}){1-2} \cmidrule(l{3pt}r{3pt}){3-6} 
  \# & \multicolumn{1}{c}{top-4 topic words} & \rotatebox{-90}{easy} & \rotatebox{-90}{normal} & \rotatebox{-90}{expert} & \rotatebox{-90}{super expert} \\
  \toprule
  \#15 & [speed, speedrun, run, seconds]  & \n[2]{topics:desc:top_n_superexpert:15:Easy_p}[100]| & \n[2]{topics:desc:top_n_superexpert:15:Normal_p}[100]| & \n[2]{topics:desc:top_n_superexpert:15:Expert_p}[100]| & \n[2]{topics:desc:top_n_superexpert:15:Super_Expert_p}[100]| \\ 
  \#13 & [jump, jumps, jumping, long]  & \n[2]{topics:desc:top_n_superexpert:13:Easy_p}[100]| & \n[2]{topics:desc:top_n_superexpert:13:Normal_p}[100]| & \n[2]{topics:desc:top_n_superexpert:13:Expert_p}[100]| & \n[2]{topics:desc:top_n_superexpert:13:Super_Expert_p}[100]| \\ 
  \#32 & [level, lol, sorry, little]  & \n[2]{topics:desc:top_n_superexpert:32:Easy_p}[100]| & \n[2]{topics:desc:top_n_superexpert:32:Normal_p}[100]| & \n[2]{topics:desc:top_n_superexpert:32:Expert_p}[100]| & \n[2]{topics:desc:top_n_superexpert:32:Super_Expert_p}[100]| \\ 
  \#56 & [practice, tricks, jumps, basic]  & \n[2]{topics:desc:top_n_superexpert:56:Easy_p}[100]| & \n[2]{topics:desc:top_n_superexpert:56:Normal_p}[100]| & \n[2]{topics:desc:top_n_superexpert:56:Expert_p}[100]| & \n[2]{topics:desc:top_n_superexpert:56:Super_Expert_p}[100]| \\ 
  \#25 & [ride, spin, run, victory]  & \n[2]{topics:desc:top_n_superexpert:25:Easy_p}[100]| & \n[2]{topics:desc:top_n_superexpert:25:Normal_p}[100]| & \n[2]{topics:desc:top_n_superexpert:25:Expert_p}[100]| & \n[2]{topics:desc:top_n_superexpert:25:Super_Expert_p}[100]| \\
  \bottomrule
  \#0 & [maker, super, bros, 11]  & \n[2]{topics:desc:top_n_easy:0:Easy_p}[100]| & \n[2]{topics:desc:top_n_easy:0:Normal_p}[100]| & \n[2]{topics:desc:top_n_easy:0:Expert_p}[100]| & \n[2]{topics:desc:top_n_easy:0:Super_Expert_p}[100]| \\ 
  \#5 & [level, level easy, easy level]  & \n[2]{topics:desc:top_n_easy:5:Easy_p}[100]| & \n[2]{topics:desc:top_n_easy:5:Normal_p}[100]| & \n[2]{topics:desc:top_n_easy:5:Expert_p}[100]| & \n[2]{topics:desc:top_n_easy:5:Super_Expert_p}[100]| \\ 
  \#30 & [world, 11, 12, 13]  & \n[2]{topics:desc:top_n_easy:30:Easy_p}[100]| & \n[2]{topics:desc:top_n_easy:30:Normal_p}[100]| & \n[2]{topics:desc:top_n_easy:30:Expert_p}[100]| & \n[2]{topics:desc:top_n_easy:30:Super_Expert_p}[100]| \\ 
  \#16 & [hard, easy, try, impossible]  & \n[2]{topics:desc:top_n_easy:16:Easy_p}[100]| & \n[2]{topics:desc:top_n_easy:16:Normal_p}[100]| & \n[2]{topics:desc:top_n_easy:16:Expert_p}[100]| & \n[2]{topics:desc:top_n_easy:16:Super_Expert_p}[100]| \\ 
  \#40 & [water, dangerous, madness, life]  & \n[2]{topics:desc:top_n_easy:40:Easy_p}[100]| & \n[2]{topics:desc:top_n_easy:40:Normal_p}[100]| & \n[2]{topics:desc:top_n_easy:40:Expert_p}[100]| & \n[2]{topics:desc:top_n_easy:40:Super_Expert_p}[100]| \\
  \bottomrule
\end{tabular}
\setlength{\tabcolsep}{6pt}
   \caption{Top-5 characterizing topics, by frequency, in titles and descriptions of \emph{super expert} (top) and \emph{easy} (bottom) levels.}
  \label{tab:desc:topics}
\end{table} 

\titledsubpar{Topics characterizing super expert levels.} The most frequent topic-word characterizing \emph{super expert} levels is
\textbf{speed}. Overall, \textbf{speed} is a topic-word in $4$ topics,
of which $3$ are characterizing for \emph{super expert}.
Similarly, \textbf{jump} is a topic-word in $14$ topics,
of which $13$ are characterizing for \emph{super expert}. All 
the $4$ topics containing \textbf{spin} as topic-word,
and all the $5$ topics containing \textbf{practice}, 
are also characterizing for \emph{super expert}. These probably indicate 
levels that let players practice and master a variety of \smm's challenging game
mechanics; in fact, these topics also include topic-words such as \textbf{jump}, \textbf{spin}, \textbf{fly}, and \textbf{tricks}.

\titledsubpar{Topics characterizing easy levels.} The most frequent topic-words characterizing 
\emph{easy} levels are very generic terms like \textbf{maker} and
\textbf{world}, which probably just means that easy levels tend to have generic titles and descriptions. 
Also self-explanatory is the second-most occurring topic-word: \textbf{easy};
among the $14$ topics that contains it, $7$ are characterizing for the \emph{easy}
\vg*{difficulty}[difficulty].
One seemingly unexpected topic-word is the number \textbf{11};
this is actually due to the way \bertopic encodes topic-words
by removing non-alphanumeric characters.
Thus, \textbf{11} actually stands for \textbf{1--1}, which is
the canonical way of referring to the first level of a multi-level world and, in particular, to the iconic \emph{World 1--1} in the original Super
Mario Bros.
Replicating such classic level in \smm, often with unique twists,
is its own sub-genre;\footnote{See for example \url{https://www.youtube.com/watch?v=PhyG0s9tJaM}}
our findings indicate that this is particularly popular with easy level---although 1--1 variants are found at all difficulties.
Other topic-words consisting of two-digit numbers (e.g., 12, 13)
have a similar explanation:
they stand for \emph{world}--\emph{level} identifiers (e.g., 1--2, 1--3).
These are either replicas of original Super Mario Bros.\ levels,
or identify levels that belong to \emph{Super Worlds}.\footnote{See \url{https://supermariomaker2.fandom.com/wiki/Super_Worlds}}
Some of the remaining topics characterizing easy levels
seem to contradict the levels' difficulty ranking,
as they include topic-words such as \textbf{hard}, \textbf{impossible},
\textbf{dangerous}, and \textbf{madness}.
A possible explanation is the makers' taste for deliberately misleading
``trolling''\footnote{\url{https://docs.google.com/document/d/13ZoqeblLs45HuEfTtsOrq6X0LAuEnA8nB721_doxE38}} titles, whereupon trivial levels are marked ``100\% impossible'' and very hard ones are titled ``easy''.






\subsection{Comments}
\label{sec:nlp:comments}

While titles and descriptions express the maker's point of view on their levels,
comments allow any players 
to voice their opinion. 
We first look at the \emph{sentiment} of level comments,
and then at their \emph{topics}.
As in \autoref{sec:nlp:titledesc},
we only consider comments written in English, as detected by \textsc{Lingua}.
To have a meaningful set of comments for each level,
we only consider levels with at least 6 comments (3\% of all levels), corresponding to a total of \n{sent:comments:N.levels} levels and 
\n{sent:comments:N.comments} comments.
Let $C(\ell)$ denote the set of comments of a level~$\ell$.

\titledpar{Sentiment.} We analyze the sentiments of the comments
by using Barbieri et al.'s~\cite{barbieri-etal-2020-tweeteval} transformer-based pipeline. For a comment $c$, the model estimates its sentiment $S(c)$
as a triple $\langle S_-(c), S_0(c), S_+(c)  \rangle$ of scores representing
the fraction of \emph{negative} $-$, \emph{neutral} $0$, and \emph{positive} $+$
sentiment, where $S_i(c) \in [0, 1]$ and $\sum_{i} S_i(c) = 1$,
$i \in \{-, 0, +\} \equiv K$.
Consider the following derived metrics,
summarized in \autoref{tab:comments:sent}:
\begin{itemize}
\item The \emph{average sentiment} $S_i(\ell)$ of $\ell$
  is the mean of $S_i(c)$ over all comments $c$ of level $\ell$.
\item The \emph{dominant sentiment} $D(c) \in K$
  is the sentiment with the highest score in $S(c)$:
  $D(c) = \argmax_{{i}} S_i(c)$.
\item $C_i(\ell) \subseteq C(\ell)$ is the set of all comments
  of $\ell$ whose dominant sentiment is $i \in K$. 
\item $\SR_i(\ell)$ is the fraction
  $|C_i(\ell)| / |C(\ell)|$
  of $\ell$'s comments whose
  dominant sentiment is $i \in K$.
\item Similarly, $\overline{S_i(X)}$ and $\overline{\SR_i(X)}$
  denote the mean of $S_i(\ell)$ and $\SR_i(\ell)$ for all levels
  of difficulty in the set $X$ of difficulties.
\end{itemize}


\begin{table}[!htb]
  \centering
  \scriptsize
    \setlength{\tabcolsep}{4pt}
\begin{tabular}{c *{4}{rr}}
  \toprule
  \multicolumn{1}{c}{\textcolor[HTML]{E7298A}{difficulty}} & \multicolumn{2}{c}{$d[S_i^x]$} & \multicolumn{2}{c}{$d[\SR_i^x]$} & \multicolumn{2}{c}{$\overline{S_i(\{x\})}$}  & \multicolumn{2}{c}{$\overline{\SR_i(\{x\})}$}\\

 $x$ & $-$ & $+$ & $-$ & $+$  & $-$ & $+$ & $-$ & $+$\\
  \cmidrule(l{3pt}r{3pt}){1-1} \cmidrule(l{3pt}r{3pt}){2-3}  \cmidrule(l{3pt}r{3pt}){4-5} \cmidrule(l{3pt}r{3pt}){6-7} \cmidrule(l{3pt}r{3pt}){8-9} 
  easy & \n[2]{d_S_i_comment:easy:neg} & \n[2]{d_S_i_comment:easy:pos} & \n[2]{d_SR_i_comment:easy:neg} & \n[2]{d_SR_i_comment:easy:pos} & \n[2]{avg_S_i_level:easy:neg} & \n[2]{avg_S_i_level:easy:pos} & \n[2]{avg_SR_i:easy:neg} & \n[2]{avg_SR_i:easy:pos}\\
  normal & \n[2]{d_S_i_comment:normal:neg} & \n[2]{d_S_i_comment:normal:pos} & \n[2]{d_SR_i_comment:normal:neg} & \n[2]{d_SR_i_comment:normal:pos} & \n[2]{avg_S_i_level:normal:neg} & \n[2]{avg_S_i_level:normal:pos} & \n[2]{avg_SR_i:normal:neg} & \n[2]{avg_SR_i:normal:pos} \\
  expert & \n[2]{d_S_i_comment:expert:neg} & \n[2]{d_S_i_comment:expert:pos} & \n[2]{d_SR_i_comment:expert:neg} & \n[2]{d_SR_i_comment:expert:pos} & \n[2]{avg_S_i_level:expert:neg} & \n[2]{avg_S_i_level:expert:pos} & \n[2]{avg_SR_i:expert:neg} & \n[2]{avg_SR_i:expert:pos}\\
  super expert & \n[2]{d_S_i_comment:superexpert:neg} & \n[2]{d_S_i_comment:superexpert:pos} & \n[2]{d_SR_i_comment:superexpert:neg} & \n[2]{d_SR_i_comment:superexpert:pos} & \n[2]{avg_S_i_level:superexpert:neg} & \n[2]{avg_S_i_level:superexpert:pos}& \n[2]{avg_SR_i:superexpert:neg} & \n[2]{avg_SR_i:superexpert:pos} \\
  \bottomrule
  \end{tabular}
\setlength{\tabcolsep}{6pt}
     \caption{An overview of the sentiments in level comments.
      The table shows the Cliff's delta of the relationship between a difficulty and all other difficulties,
      as well as the mean of the average sentiment $S_i(\ell)$
      and of the fraction of dominant sentiment $\SR_i(\ell)$
      over all levels $\ell$ of each difficulty $x$.}
  \label{tab:comments:sent}
\end{table}

A trend visible in \autoref{tab:comments:sent}
is that \emph{super expert} level comments
display a higher negative average sentiment than other difficulties;
this holds both for the $S_{-}$ and the $\SR_{-}$ metrics,
that is whether we aggregate by average or by dominant sentiment.
To quantify this observation,
we compute Cliff's delta---a non-parametric effect size,
suitable to quantify how often the values
in one set are larger than the values in another, independent set,
without assumptions about their underlying distributions.
Let $d[S_i^x]$ denote Cliff's delta of the differences
between $\overline{S_i(\{x\})}$ and $\overline{S_i(\{y \neq x\})}$, i.e., between the average $S_i$ for all levels of difficulty $x$ and the average $S_i$ for all other levels;
similarly, $d[\SR_i^x]$ denotes Cliff's delta of the corresponding difference
of metric $\SR_i$.
\autoref{tab:comments:sent} shows that
$d[S_-^{\text{super expert}}] = \n[2]{d_S_i_comment:superexpert:neg}$
and $d[\SR_-^{\text{super expert}}] = \n[2]{d_SR_i_comment:superexpert:neg}$,
Such effect sizes are usually considered \emph{small} but not negligible~\cite{Romano:2006};\footnote{Null-hypothesis statistical testing is uninformative in this case (possibly in general~\cite{pvalue-cohen}),
  since the sheer amount of data leads to minuscule $p$-values.
}
in contrast, $d[S_i^x]$ and $d[\SR_i^x]$ are \emph{negligible}
for all other difficulties $x$ other than \emph{super expert},
and in all ratings corresponding to positive sentiment, 
which supports our observation that players of super expert
 levels tend to express more negative sentiments.





\titledpar{Topics.}
We analyzed English user comments by applying \bertopic as in \autoref{sec:nlp:titledesc},
aggregating comment topic occurrences by \emph{level};
thus, a topic $t$ has occurrence frequency $\tau\%$ for a certain difficulty $x$
if $\tau\%$ of the $x$-difficulty levels include at least one comment
with topic $t$.
\autoref{tab:comments:topics}
lists the top-5 characterizing topics for the
\emph{super expert} and \emph{easy} difficulties.




\begin{table}[h]
  \centering
  \scriptsize
    \setlength{\tabcolsep}{4pt}
\begin{tabular}{llrrrrc}
  \toprule
  \multicolumn{2}{c}{topic} &
  \multicolumn{4}{c}{frequency per \textcolor[HTML]{E7298A}{difficulty}} \\
  \cmidrule(l{3pt}r{3pt}){1-2} \cmidrule(l{3pt}r{3pt}){3-6} 
  \# & \multicolumn{1}{c}{top-4 topic words} & \multicolumn{1}{c}{\rotatebox{-90}{easy}} & \multicolumn{1}{c}{\rotatebox{-90}{normal}} & \multicolumn{1}{c}{\rotatebox{-90}{expert}} & \multicolumn{1}{c}{\rotatebox{-90}{super expert}} \\
  \toprule
  \#0 & [level, great level, good level]  & \n[2]{topics:comm:top_n_superexpert:0:Easy_p}[100]| & \n[2]{topics:comm:top_n_superexpert:0:Normal_p}[100]| & \n[2]{topics:comm:top_n_superexpert:0:Expert_p}[100]| & \n[2]{topics:comm:top_n_superexpert:0:Super_Expert_p}[100]| \\ 
  \#5 & [hard, easy, beat, challenge]  & \n[2]{topics:comm:top_n_superexpert:5:Easy_p}[100]| & \n[2]{topics:comm:top_n_superexpert:5:Normal_p}[100]| & \n[2]{topics:comm:top_n_superexpert:5:Expert_p}[100]| & \n[2]{topics:comm:top_n_superexpert:5:Super_Expert_p}[100]| \\ 
  \#10 & [jump, spin, jumping, jumped]  & \n[2]{topics:comm:top_n_superexpert:10:Easy_p}[100]| & \n[2]{topics:comm:top_n_superexpert:10:Normal_p}[100]| & \n[2]{topics:comm:top_n_superexpert:10:Expert_p}[100]| & \n[2]{topics:comm:top_n_superexpert:10:Super_Expert_p}[100]| \\ 
  \#50 & [shell, jump, throw, double]  & \n[2]{topics:comm:top_n_superexpert:50:Easy_p}[100]| & \n[2]{topics:comm:top_n_superexpert:50:Normal_p}[100]| & \n[2]{topics:comm:top_n_superexpert:50:Expert_p}[100]| & \n[2]{topics:comm:top_n_superexpert:50:Super_Expert_p}[100]| \\ 
  \#38 & [troll, bully, mad, lad]  & \n[2]{topics:comm:top_n_superexpert:38:Easy_p}[100]| & \n[2]{topics:comm:top_n_superexpert:38:Normal_p}[100]| & \n[2]{topics:comm:top_n_superexpert:38:Expert_p}[100]| & \n[2]{topics:comm:top_n_superexpert:38:Super_Expert_p}[100]| \\
  \bottomrule
  \#1 & [mario, toad, bros, maker]  & \n[2]{topics:comm:top_n_easy:1:Easy_p}[100]| & \n[2]{topics:comm:top_n_easy:1:Normal_p}[100]| & \n[2]{topics:comm:top_n_easy:1:Expert_p}[100]| & \n[2]{topics:comm:top_n_easy:1:Super_Expert_p}[100]| \\ 
  \#2 & [nintendo, switch, minecraft]  & \n[2]{topics:comm:top_n_easy:2:Easy_p}[100]| & \n[2]{topics:comm:top_n_easy:2:Normal_p}[100]| & \n[2]{topics:comm:top_n_easy:2:Expert_p}[100]| & \n[2]{topics:comm:top_n_easy:2:Super_Expert_p}[100]| \\ 
  \#3 & [course, great course, fun course]  & \n[2]{topics:comm:top_n_easy:3:Easy_p}[100]| & \n[2]{topics:comm:top_n_easy:3:Normal_p}[100]| & \n[2]{topics:comm:top_n_easy:3:Expert_p}[100]| & \n[2]{topics:comm:top_n_easy:3:Super_Expert_p}[100]| \\ 
  \#4 & [awesome, good job, thanks]  & \n[2]{topics:comm:top_n_easy:4:Easy_p}[100]| & \n[2]{topics:comm:top_n_easy:4:Normal_p}[100]| & \n[2]{topics:comm:top_n_easy:4:Expert_p}[100]| & \n[2]{topics:comm:top_n_easy:4:Super_Expert_p}[100]| \\ 
  \#8 & [brain, eyes, pain, dad]  & \n[2]{topics:comm:top_n_easy:8:Easy_p}[100]| & \n[2]{topics:comm:top_n_easy:8:Normal_p}[100]| & \n[2]{topics:comm:top_n_easy:8:Expert_p}[100]| & \n[2]{topics:comm:top_n_easy:8:Super_Expert_p}[100]| \\ 
  \bottomrule
\end{tabular}
\setlength{\tabcolsep}{6pt}
   \caption{Top-5 characterizing topics, by frequency, in comments of \emph{super expert} (top) and \emph{easy} (bottom) levels.}
  \label{tab:comments:topics}
\end{table} 

\titledsubpar{Comment topics characterizing super expert levels.}
The most frequently occurring characterizing topic in super expert levels
seems to denote appreciation (e.g., \textbf{great}/\textbf{good} level);
indeed, the average $+$ sentiment for comments
with this topic is \n[2]{topics:comm:0:sent_pos:avg}, which is comparatively high.
In contrast,
topic 38 indicates dislike,
and the average $-$ sentiment for comments with this topic
is \n[2]{topics:comm:38:sent_neg:avg},
which is also above average.
This finding complements the previous observation about negative sentiments
in super expert comments:
while users are frustrated by trolly or gratuitously hard levels,
they arguably appreciate when the difficulty is fair
and determines a challenging but satisfying level.
The other characterizing topics of super expert level comments
are in line with \autoref{sec:nlp:titledesc}'s analysis,
showing frequent mention of topic-words that suggest
challenging game mechanic---such as \textbf{shell} \textbf{jumps}
and \textbf{double}/triple jumps.


\titledsubpar{Comment topics characterizing easy levels.}
Topics \#3 and \#4 in \autoref{tab:comments:topics}
seem to indicate generic user appreciation of a level;
in fact the average $+$ sentiment for comments with these topics
are \n[2]{topics:comm:3:sent_pos:avg} and \n[2]{topics:comm:4:sent_pos:avg}
respectively---both clearly above average.
In contrast,
topic \#8 leans towards negative;
its average negative sentiment is
\n[2]{topics:comm:8:sent_neg:avg},
clearly above the average negative sentiment of \emph{easy} levels.
Topic-words such as \textbf{brain}, \textbf{eyes}, and \textbf{pain}
suggest that the most common criticism of easy levels
targets those that make an unnecessary, excessive usage
of flashy
effects,\footnote{\url{https://supermariomaker2.fandom.com/wiki/Sound_Effects}}
which can significantly deteriorate the user experience.
Finally, topics \#1 and \#2 seem generically positive (or possibly neutral) comments.
However, topic-word \textbf{Minecraft} stands out,
which may indicate attempts at translating some of Minecraft's
features as a \smm level;
the stronger association with easy levels
might indicate that such attempts tend to be uninteresting
from the perspective of platforming level design.




